Direct Quantization for Training Highly Accurate Low Bit-width Deep Neural Networks

This paper proposes two novel techniques to train deep convolutional neural networks with low bit-width weights and activations. First, to obtain low bit-width weights, most existing methods obtain the quantized weights by performing quantization on the full-precision network weights. However, this approach would result in some mismatch: the gradient descent updates full-precision weights, but it does not update the quantized weights. To address this issue, we propose a novel method that enables {direct} updating of quantized weights {with learnable quantization levels} to minimize the cost function using gradient descent. Second, to obtain low bit-width activations, existing works consider all channels equally. However, the activation quantizers could be biased toward a few channels with high-variance. To address this issue, we propose a method to take into account the quantization errors of individual channels. With this approach, we can learn activation quantizers that minimize the quantization errors in the majority of channels. Experimental results demonstrate that our proposed method achieves state-of-the-art performance on the image classification task, using AlexNet, ResNet and MobileNetV2 architectures on CIFAR-100 and ImageNet datasets.

==> [IJCAI20_camera_ready] Network quantization/ijcai20bib <==


@InProceedings{zhou:2018,
author = {Yiren Zhou and Seyed-Mohsen Moosavi-Dezfooli and  Ngai-Man Cheung and Pascal Frossard},
title = {Adaptive Quantization for Deep Neural Network},
booktitle = {AAAI},
year = {2018},
pages={4596--4604},
}


@InProceedings{Yang_2019_CVPR,
author = {Yang, Jiwei and Shen, Xu and Xing, Jun and Tian, Xinmei and Li, Houqiang and Deng, Bing and Huang, Jianqiang and Hua, Xian-sheng},
title = {Quantization Networks},
booktitle = {CVPR},
year = {2019},
pages={7300-7308},
}

@INPROCEEDINGS{RBCN,
  title={{Rectified Binary Convolutional Networks for Enhancing the Performance of 1-bit DCNNs}},
  author={Chunlei Liu and Wenrui Ding and Xin Xia and Yuan Hu and Baochang Zhang and Jianzhuang Liu and Bohan Zhuang and Guodong Guo},
  booktitle={IJCAI},
  year={2019},
  pages= {854--860},
}

@INPROCEEDINGS{BBG, 
author={M. {Shen} and X. {Liu} and R. {Gong} and K. {Han}},
booktitle={ICASSP}, 
title={Balanced Binary Neural Networks with Gated Residual}, 
year={2020}}

@INPROCEEDINGS{MobileNetV2, 
author={Mark Sandler and Andrew Howard and Menglong Zhu and Andrey Zhmoginov and Liang-Chieh Chen},
booktitle={CVPR}, 
title={{MobileNetV2: Inverted Residuals and Linear Bottlenecks}}, year={2018}, 
pages={4510-4520},
}



@inproceedings{TernGrad,
 author = {Wen, Wei and Xu, Cong and Yan, Feng and Wu, Chunpeng and Wang, Yandan and Chen, Yiran and Li, Hai},
 title = {TernGrad: Ternary Gradients to Reduce Communication in Distributed Deep Learning},
 booktitle = {NIPS},
 year = {2017},
} 

@inproceedings{pcnn,
  title={Projection Convolutional Neural Networks for 1-bit CNNs via Discrete Back Propagation},
  author={Jiaxin, Gu and Ce, Li and Baochang, Zhang and Jungong, Han and Xianbin, Cao and Jianzhuang, Liu and David, Doermann},
  booktitle={AAAI},
  year={2019}
}

@inproceedings{bonn,
  title={{Bayesian Optimized 1-bit CNNs}},
  author={Gu, Jiaxin and Zhao, Junhe and Jiang, Xiaolong and Zhang, Baochang and Liu Jianzhuang and Guo, Guodong and Ji, Rongrong},
  booktitle={ICCV},
  year={2019},
  pages={4909-4917}
}

@InProceedings{dsq,
    title={Differentiable Soft Quantization: Bridging Full-Precision and Low-Bit Neural Networks},
    author={Gong, Ruihao and Xianglong Liu and Shenghu Jiang and Tianxiang Li and Peng Hu and Jiazhen Lin and Fengwei Yu and Junjie Yan},
    year={2019},
    pages = {4852-4861},
    booktitle={ICCV},
}

@article{wage,
  author    = {Shuang Wu and
               Guoqi Li and
               Feng Chen and
               Luping Shi},
  title     = {Training and Inference with Integers in Deep Neural Networks},
  booktitle = {ICLR},
  year      = {2018},
}


@InProceedings{MorphNet,
author = {Gordon, Ariel and Eban, Elad and Nachum, Ofir and Chen, Bo and Wu, Hao and Yang, Tien-Ju and Choi, Edward},
title = {MorphNet: Fast \& Simple Resource-Constrained Structure Learning of Deep Networks},
booktitle = {CVPR},
year = {2018}
}

@inproceedings{netcompress_vec_quant,
  author    = {Yunchao Gong and
               Liu Liu and
               Ming Yang and
               Lubomir D. Bourdev},
  title     = {Compressing Deep Convolutional Networks using Vector Quantization},
  booktitle={ICLR Workshop},
  year={2015}
}

@inproceedings{TNN_truncatedGauusianApprox,
  author    = {Zhezhi He and
               Deliang Fan},
  title     = {{Simultaneously Optimizing Weight and Quantizer of Ternary Neural Network
               using Truncated Gaussian Approximation}},
  booktitle={CVPR},
  year={2019}
}


@inproceedings{groupnet,
  author    = {Bohan Zhuang and
               Chunhua Shen and
               Mingkui Tan and
               Lingqiao Liu and
               Ian D. Reid},
  title     = {{Structured Binary Neural Networks for Accurate Image Classification and Semantic Segmentation}},
    booktitle={CVPR},
  year={2019},
  pages={413--422},
}

@inproceedings{binary_ensemble_NN,
  author    = {Shilin Zhu and
               Xin Dong and
               Hao Su},
  title     = {{Binary Ensemble Neural Network: More Bits per Network or More Networks per Bit?}},
  booktitle={CVPR},
  year={2019}
}


@inproceedings{CBCN,
  title={{Circulant Binary Convolutional Networks: Enhancing the Performance of 1-bit DCNNs with Circulant Back Propagation}},
  author={Liu, Chunlei and Ding, Wenrui and Gu, Jiaxin and Zhang, Baochang and Ji, Rongrong and Liu, Jianzhuang},
  booktitle={CVPR},
  year={2019}
}

@InProceedings{QIL,
author = {Jung, Sangil and Son, Changyong and Lee, Seohyung and Son, Jinwoo and Han, Jae-Joon and Kwak, Youngjun and Hwang, Sung Ju and Choi, Changkyu},
title = {Learning to Quantize Deep Networks by Optimizing Quantization Intervals With Task Loss},
booktitle = {CVPR},
year = {2019},
pages = {4350--4359},
}

@InProceedings{OQI,
  author    = {Sangil Jung and
               Changyong Son and
               Seohyung Lee and
               JinWoo Son and
               Youngjun Kwak and
               Jae{-}Joon Han and
               Changkyu Choi},
  title     = {{Joint Training of Low-Precision Neural Network with Quantization Interval Parameters}},
booktitle = {CVPR},
  year      = {2019},
}

@InProceedings{bi-real,
author = {Liu, Zechun and Wu, Baoyuan and Luo, Wenhan and Yang, Xin and Liu, Wei and Cheng, Kwang-Ting},
title = {{Bi-Real Net: Enhancing the Performance of 1-bit CNNs with Improved Representational Capability and Advanced Training Algorithm}},
booktitle = {ECCV},
year = {2018},
pages={747--763},
}

@incollection{discrimiation_aware_prunning,
title = {{Discrimination-aware Channel Pruning for Deep Neural Networks}},
author = {Zhuang, Zhuangwei and Tan, Mingkui and Zhuang, Bohan and Liu, Jing and Guo, Yong and Wu, Qingyao and Huang, Junzhou and Zhu, Jinhui},
booktitle = {NIPS},
pages = {875--886},
year = {2018},
}


@incollection{NIPS2017_6638,
title = {{Towards Accurate Binary Convolutional Neural Network}},
author = {Lin, Xiaofan and Zhao, Cong and Pan, Wei},
booktitle = {NIPS},
pages = {345--353},
year = {2017},
}


@InProceedings{LessIsMore,
author="Zhou, Hao
and Alvarez, Jose M.
and Porikli, Fatih",
editor="Leibe, Bastian
and Matas, Jiri
and Sebe, Nicu
and Welling, Max",
title={{Less Is More: Towards Compact CNNs}},
booktitle="ECCV",
year="2016",
}

@article{log_data_represent,
  author    = {Daisuke Miyashita and
               Edward H. Lee and
               Boris Murmann},
  title     = {{Convolutional Neural Networks using Logarithmic Data Representation}},
  journal   = {CoRR},
  volume    = {abs/1603.01025},
  year      = {2016},
}

@InProceedings{explicit_lossaware,
author = {Zhou, Aojun and Yao, Anbang and Wang, Kuan and Chen, Yurong},
title = {{Explicit Loss-Error-Aware Quantization for Low-Bit Deep Neural Networks}},
booktitle = {CVPR},
month = {June},
year = {2018}
}

@article{dropout,
 author = {Srivastava, Nitish and Hinton, Geoffrey and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
 title = {{Dropout: A Simple Way to Prevent Neural Networks from Overfitting}},
 journal = {JMLR},
 issue_date = {January 2014},
 volume = {15},
 number = {1},
 month = jan,
 year = {2014},
 pages = {1929--1958},
} 


@InProceedings{xavier_init,
  title = 	 {Understanding the difficulty of training deep feed-forward neural networks},
  author = 	 {Xavier, Glorot and Yoshua, Bengio},
  booktitle = 	 {AISTATS},
  year = 	 {2010},
}

@article{QNN,
 author = {Hubara, Itay and Courbariaux, Matthieu and Soudry, Daniel and El-Yaniv, Ran and Bengio, Yoshua},
 title = {{Quantized Neural Networks: Training Neural Networks with Low Precision Weights and Activations}},
 journal = {JMLR},
 year = {2017},
 pages = {6869–6898},
 volume = {18},
number = {1},
} 

@inproceedings{INQ,
title={{Incremental Network Quantization: Towards Lossless CNNs with Low-Precision Weights}},
author={Aojun, Zhou and Anbang, Yao and Yiwen, Guo and Lin, Xu and Yurong, Chen},
booktitle={ICLR},
year={2017},
}

@InProceedings{DL_limited_num_precision,
  title = 	 {{Deep Learning with Limited Numerical Precision}},
  author = 	 {Suyog Gupta and Ankur Agrawal and Kailash Gopalakrishnan and Pritish Narayanan},
  booktitle = 	 {ICML},
  year = 	 {2015},
  pages = {1737–1746},
}

@inproceedings{NN_few_mul,
  title={{Neural Networks with Few Multiplications}},
  author={Zhouhan Lin and Matthieu Courbariaux and Roland Memisevic and Yoshua Bengio},
 booktitle = {ICML},
 year = {2016},
}

@inproceedings{fix_point_quant,
 author = {Darryl D. Lin and Sachin S. Talathi and V. Sreekanth Annapureddy},
 title = {{Fixed Point Quantization of Deep Convolutional Networks}},
 booktitle = {ICML},
 year = {2016},
 pages = {2849–2858},
} 

@incollection{BinaryConnect,
title = {{BinaryConnect: Training Deep Neural Networks with binary weights during propagations}},
author = {Courbariaux, Matthieu and Bengio, Yoshua and David, Jean-Pierre},
booktitle = {NIPS},
pages = {3123--3131},
year = {2015},
}

@inproceedings{8bit_parallel,
  author    = {Tim Dettmers},
  title     = {8-BIT APPROXIMATIONS FOR PARALLELISM IN DEEP LEARNING},
  booktitle={ICLR},
  year      = {2016},
}

@inproceedings{TWN,
  author    = {Fengfu Li and
               Bin Liu},
  title     = {Ternary Weight Networks},
  booktitle={ICLR},
  year      = {2017},
}

@inproceedings{batch_norm,
 author = {Ioffe, Sergey and Szegedy, Christian},
 title = {Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift},
 booktitle = {ICML},
 year = {2015},
 pages = {448–456},
} 

@InProceedings{lossaware17,
	title={Loss-aware Binarization of Deep Networks},
	author={Hou, Lu and Yao, Quanming and Kwok, James T.},
	booktitle={ICLR},
	year={2017}
}

@inproceedings{lossaware,
title={Loss-aware Weight Quantization of Deep Networks},
author={Lu Hou and James T. Kwok},
booktitle={ICLR},
year={2018},
}

@inproceedings{FasterGP,
  title={{Faster gaze prediction with dense networks and Fisher pruning}},
  author={Lucas Theis and Iryna Korshunova and Alykhan Tejani and Ferenc Husz{\'a}r},
 booktitle = {ECCV},
month = {June},
year = {2018}
}

@InProceedings{Learning-Compression,
author = {Carreira-Perpinan, Miguel A. and Idelbayev, Yerlan},
title = {{“Learning-Compression” Algorithms for Neural Net Pruning}},
booktitle = {CVPR},
year = {2018}
}

@inproceedings{NetworkSlimming,
	title = {Learning Efficient Convolutional Networks through Network Slimming},
	author = {Liu, Zhuang and Li, Jianguo and Shen, Zhiqiang and Huang, Gao and Yan, Shoumeng and Zhang, Changshui},
	booktitle = {ICCV},
	year = {2017}
}

@InProceedings{nips,
author = {Yu, Ruichi and Li, Ang and Chen, Chun-Fu and Lai, Jui-Hsin and I. Morariu, Vlad and Han, Xintong and Gao, Mingfei and Lin, Ching-Yung and Davis, Larry},
year = {2018},
booktitle = {CVPR},
title = {{NISP: Pruning Networks using Neuron Importance Score Propagation}}
}

@InProceedings{ThiNet,
  author={Jian-Hao Luo, Jianxin Wu, and Weiyao Lin},
  title={{ThiNet: A Filter Level Pruning Method for Deep Neural Network Compression}},
  booktitle={ICCV},
  year = {2017},
}

@InProceedings{channel_pruning,
author = {He, Yihui and Zhang, Xiangyu and Sun, Jian},
title = {{Channel Pruning for Accelerating Very Deep Neural Networks}},
booktitle = {ICCV},
year = {2017}
}


@inproceedings{LBWC,
 author = {Han, Song and Pool, Jeff and Tran, John and Dally, William J.},
 title = {{Learning Both Weights and Connections for Efficient Neural Networks}},
 booktitle = {NIPS},
 year = {2015},
} 

@article{accelerateCNN,
 author = {Zhang, Xiangyu and Zou, Jianhua and He, Kaiming and Sun, Jian},
 title = {Accelerating Very Deep Convolutional Networks for Classification and Detection},
 journal = {IEEE TPAMI},
 issue_date = {October 2016},
 volume = {38},
 number = {10},
 year = {2016},
 pages = {1943--1955},
} 


@inproceedings{tensorizing,
 author = {Novikov, Alexander and Podoprikhin, Dmitry and Osokin, Anton and Vetrov, Dmitry},
 title = {Tensorizing Neural Networks},
 booktitle = {NIPS},
 year = {2015},
} 

@inproceedings{CP-Decomposition,
author = {Lebedev, Vadim and Ganin, Yaroslav and Rakhuba, Maksim and Oseledets, Ivan and Lempitsky, Victor},
year = {2015},
booktitle = {ICLR},
title = {{Speeding-up Convolutional Neural Networks Using Fine-tuned CP-Decomposition}},
}

@inproceedings{low_rank_expansion,
  title={Speeding up Convolutional Neural Networks with Low Rank Expansions},
  author={Max Jaderberg and Andrea Vedaldi and Andrew Zisserman},
  booktitle={BMVC},
  year={2014},
}

@inproceedings{linear_structure,
 author = {Denton, Emily and Zaremba, Wojciech and Bruna, Joan and LeCun, Yann and Fergus, Rob},
 title = {{Exploiting Linear Structure Within Convolutional Networks for Efficient Evaluation}},
 booktitle = {NIPS},
 year = {2014},
} 


@inproceedings{predict_param,
 author = {Denil, Misha and Shakibi, Babak and Dinh, Laurent and Ranzato, Marc'Aurelio and de Freitas, Nando},
 title = {{Predicting Parameters in Deep Learning}},
 booktitle = {NIPS},
 year = {2013},
} 

@article{GoogLeNet,
  title={Going deeper with convolutions},
  author={Christian Szegedy and Wei Liu and Yangqing Jia and Pierre Sermanet and Scott E. Reed and Dragomir Anguelov and Dumitru Erhan and Vincent Vanhoucke and Andrew Rabinovich},
  journal={CVPR},
  year={2015},
}

@inproceedings{MobileNets,
author = {G. Howard, Andrew and Zhu, Menglong and Chen, Bo and Kalenichenko, Dmitry and Wang, Weijun and Weyand, Tobias and Andreetto, Marco and Adam, Hartwig},
year = {2017},
title = {{MobileNets: Efficient Convolutional Neural Networks for Mobile Vision Applications}},
booktitle = {CVPR},
}

@inproceedings{ShuffleNet,
author = {Zhang, Xiangyu and Zhou, Xinyu and Lin, Mengxiao and Sun, Jian},
year = {2017},
title = {{ShuffleNet: An Extremely Efficient Convolutional Neural Network for Mobile Devices}},
booktitle = {CVPR},
}

@article{SqueezeNet,
  author    = {Forrest N. Iandola and
               Matthew W. Moskewicz and
               Khalid Ashraf and
               Song Han and
               William J. Dally and
               Kurt Keutzer},
  title     = {{SqueezeNet: AlexNet-level accuracy with 50x fewer parameters and {\textless}1MB model size}},
  journal   = {CoRR},
  volume    = {abs/1602.07360},
  year      = {2016},
}


@inproceedings{net_in_net,
  author    = {Min Lin and
               Qiang Chen and
               Shuicheng Yan},
  title     = {Network In Network},
    booktitle = {ICLR},
  year={2014}
}

@inproceedings{TTQ,
  title={{Trained Ternary Quantization}},
  author={Zhu, Chenzhuo and Han, Song and Mao, Huizi and Dally, William J},
  booktitle = {ICLR},
  year={2017}
}

@inproceedings{LQNets,
    author = {Zhang, Dongqing and Yang, Jiaolong and Ye, Dongqiangzi and Hua, Gang},
    title = {{LQ-Nets: Learned Quantization for Highly Accurate and Compact Deep Neural Networks}},
    booktitle = {ECCV},
    year = {2018},
    pages={373--390},
}

@article{TwoStepQF,
  title={{Two-Step Quantization for Low-bit Neural Networks}},
  author={Peisong Wang and Qinghao Hu and Yifan Zhang and Chunjie Zhang and Yang Liu and Jian Cheng},
  journal={CVPR},
  year={2018},
}

@inproceedings{hwgq,
  author = {Zhaowei Cai and Xiaodong He and Jian Sun and Nuno Vasconcelos},
  Title = {{Deep Learning with Low Precision by Half-wave Gaussian Quantization}},
  booktitle = {CVPR},
  pages={5918-5926},
  Year  = {2017}
}

@inproceedings{HORQ,
author = {Li, Zefan and Ni, Bingbing and Zhang, Wenjun and Yang, Xiaokang and Gao, Wen},
year = {2017},
title = {{Performance Guaranteed Network Acceleration via High-Order Residual Quantization}},
booktitle = {ICCV},
pages={2584-2592},
}

@InProceedings{BinaryNet,
author = {Wei Tang and Gang Hua and Liang Wang},
title = {{How to Train a Compact Binary Neural Network with High Accuracy?}},
booktitle = {AAAI},
year = {2017},
pages={2625--2631},
}

@InProceedings{tbn,
author = {Wan, Diwen and Shen, Fumin and Liu, Li and Zhu, Fan and Qin, Jie and Shao, Ling and Tao Shen, Heng},
title = {{TBN: Convolutional Neural Network with Ternary Inputs and Binary Weights}},
booktitle = {ECCV},
year = {2018},
pages={322--339},
}

@InProceedings{BNN,
  title={{BinaryNet: Training Deep Neural Networks with Weights and Activations Constrained to +1 or -1}},
  author={Matthieu Courbariaux and Yoshua Bengio},
  booktitle={NIPS},
  year={2016},
}

@inproceedings{tnn,
author = {Alemdar, Hande and Leroy, Vincent and Prost-Boucle, Adrien and Pétrot, Frédéric},
year = {2017},
title = {{Ternary neural networks for resource-efficient AI applications}},
booktitle = {IJCNN}
}

@InProceedings{xnor_net,
author="Rastegari, Mohammad and Ordonez, Vicente and Redmon, Joseph and Farhadi, Ali",
title={{XNOR-Net: ImageNet Classification Using Binary Convolutional Neural Networks}},
booktitle="ECCV",
year="2016",
pages="525--542",
}

@INPROCEEDINGS{entropy_penalize, 
author={Gabriel Pereyra and George Tucker and Jan Chorowski and Łukasz Kaiser and Geoffrey Hinton}, 
booktitle={ICLR Workshop}, 
title={Regularizing neural networks by penalizing confident output distributions}, 
year={2017}, }


@INPROCEEDINGS{weighted_entropy, 
author={Eunhyeok Park and Junwhan Ahn and Sungjoo Yoo}, 
booktitle={CVPR}, 
title={Weighted-Entropy-Based Quantization for Deep Neural Networks}, 
year={2017}, 
pages={5456--5464},
}

@inproceedings{DeepCompression,
author = {Han, Song and Mao, Huizi and Dally, William},
year = {2016},
booktitle={ICLR},
title = {{Deep Compression: Compressing Deep Neural Networks with Pruning, Trained Quantization and Huffman Coding}}
}

@inproceedings{LearningWeightConnect,
  title={Learning both Weights and Connections for Efficient Neural Networks},
  author={Song Han and Jeff Pool and John Tran and William J. Dally},
  booktitle={NIPS},
  year={2015}
}

@incollection{soft2hard,
title = {Soft-to-Hard Vector Quantization for End-to-End Learning Compressible Representations},
author = {Agustsson, Eirikur and Mentzer, Fabian and Tschannen, Michael and Cavigelli, Lukas and Timofte, Radu and Benini, Luca and Gool, Luc V},
booktitle = {NIPS},
year = {2017},
}

@inproceedings{BinarizedNN,
  title={Binarized Neural Networks},
  author={Itay Hubara and Matthieu Courbariaux and Daniel Soudry and Ran El-Yaniv and Yoshua Bengio},
  booktitle={NIPS},
  year={2016}
}

@article{STE,
author = {Hinton, Geoffreye},
year = {2012},
title = {Neural networks for machine learning},
journal = {Coursera, video lectures}
}

@article{STE1,
  title={Estimating or Propagating Gradients Through Stochastic Neurons for Conditional Computation},
  author={Yoshua Bengio and Nicholas L{\'e}onard and Aaron C. Courville},
  journal={CoRR},
  year={2013},
  volume={abs/1308.3432}
}

@book{info_theory,
 author = {Cover, Thomas M. and Thomas, Joy A.},
 title = {Elements of Information Theory},
 year = {2006},
 isbn = {0471241954},
 publisher = {Wiley-Interscience},
} 

@inproceedings{ternary_quant,
  title={Trained Ternary Quantization},
  author={Zhu, Chenzhuo and Han, Song and Mao, Huizi and Dally, William J},
  booktitle={ICLR},
  year={2017}
}

@inproceedings{imagenet,
AUTHOR = {Jia Deng and Wei Dong and Richard Socher and Li-Jia Li and {Kai Li} and {Li Fei-Fei}},
TITLE = {{ImageNet: A Large-Scale Hierarchical Image Database}},
BOOKTITLE = {CVPR},
YEAR = {2009},
pages={248-255}
}
        

@TECHREPORT{cifar10,
    author = {Alex Krizhevsky},
    title = {Learning multiple layers of features from tiny images},
    institution = {University of Toronto},
    year = {2009}
}

@INPROCEEDINGS{8099498, 
author={X. Yu and T. Liu and X. Wang and D. Tao}, 
booktitle={CVPR}, 
title={On Compressing Deep Models by Low Rank and Sparse Decomposition}, 
year={2017}, 
}

@article{dorefa,
  author    = {Shuchang Zhou and Yuxin Wu and Zekun Ni and Xinyu Zhou and He Wen and Yuheng Zou},
  title     = {{DoReFa-Net: Training Low Bitwidth Convolutional Neural Networks with Low Bitwidth Gradients}},
  journal   = {CoRR},
  volume    = {abs/1606.06160},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.06160},
}

@inproceedings{guidedQuantize,
  title={{Towards Effective Low-Bitwidth Convolutional Neural Networks}},
  author={Bohan Zhuang and Chunhua Shen and Mingkui Tan and Lingqiao Liu and Ian D. Reid},
  booktitle={CVPR},
  year={2018},
  pages={7920--7928},
}


@inproceedings{spectralnet,
title={SpectralNet: Spectral Clustering using Deep Neural Networks},
author={Uri Shaham and Kelly Stanton and Henry Li and Ronen Basri and Boaz Nadler and Yuval Kluger},
booktitle={ICLR},
year={2018},
}

@incollection{rank_manifold,
title = {Ranking on Data Manifolds},
author = {Zhou, Dengyong and Weston, Jason and Gretton, Arthur and Bousquet, Olivier and Sch\"{o}lkopf, Bernhard},
booktitle = {NIPS},
year = {2004},
}

@article{diff_web,
author = {Page, Lawrence and Brin, Sergey and Motwani, Rajeev and Winograd, Terry},
year = {1998},
month = {11},
title = {The PageRank Citation Ranking: Bringing Order to the Web}
}

@INPROCEEDINGS{diff_revisit, 
author={M. Donoser and H. Bischof}, 
booktitle={CVPR}, 
title={Diffusion Processes for Retrieval Revisited}, 
year={2013}, 
}

@inproceedings{diff_orig,
author = {Zhou, Dengyong and Bousquet, Olivier and Lal, Thomas Navin and Weston, Jason and Sch\"{o}lkopf, Bernhard},
title = {Learning with Local and Global Consistency},
booktitle = {NIPS},
year = {2003},
location = {Whistler, British Columbia, Canada},
} 


@ARTICLE{DRSCH, 
author={R. Zhang and L. Lin and R. Zhang and W. Zuo and L. Zhang}, 
journal={IEEE TIP}, 
title={Bit-Scalable Deep Hashing With Regularized Similarity Learning for Image Retrieval and Person Re-Identification}, 
year={2015}, 
volume={24}, 
number={12}, 
}

@inproceedings{hashnet,
title={HashNet: Deep Learning to Hash by Continuation},
author={Cao, Zhangjie and Long, Mingsheng and Wang, Jianmin and Yu, Philip S},
booktitle = {CVPR},
year={2018}
}

@inproceedings{doersch2015unsupervised,
  title = {Unsupervised Visual Representation Learning by Context Prediction},
  author = {Doersch, Carl and Gupta, Abhinav and Efros, Alexei A.},
  booktitle = {ICCV},
  year = {2015}
}

@inproceedings{pathakCVPR16context,
    Author = {Pathak, Deepak and
    Kr\"ahenb\"uhl, Philipp and
    Donahue, Jeff and
    Darrell, Trevor and
    Efros, Alexei},
    Title = {Context Encoders:
    Feature Learning by Inpainting},
    booktitle = {CVPR},
    Year = {2016}
}

@article{FM_gan,
  title={Adversarial Text Generation via Feature-Mover's Distance},
  author={Liqun Chen and Shuyang Dai and Chenyang Tao and Dinghan Shen and Zhe Gan and Haichao Zhang and Yizhe Zhang and Lawrence Carin},
  booktitle={NIPS},
  year={2018}
}

@inproceedings{BGAN,
  title={Binary Generative Adversarial Networks for Image Retrieval},
  author={Jingkuan Song and Tao He and Lianli Gao and Xing Xu and Alan Hanjalic and Heng Tao Shen},
  booktitle={AAAI},
  year={2018}
}

@InProceedings{codes,
author="Douze, Matthijs
and J{\'e}gou, Herv{\'e}
and Perronnin, Florent",
editor="Leibe, Bastian
and Matas, Jiri
and Sebe, Nicu
and Welling, Max",
title="Polysemous Codes",
booktitle="ECCV",
year="2016",
}



@incollection{DGH,
title = {Discrete Graph Hashing},
author = {Liu, Wei and Mu, Cun and Kumar, Sanjiv and Chang, Shih-Fu},
booktitle = {NIPS},
year = {2014},
}

@INPROCEEDINGS{FSH, 
author={H. Liu and R. Ji and Y. Wu and F. Huang and B. Zhang}, 
booktitle={CVPR}, 
title={Cross-Modality Binary Code Learning via Fusion Similarity Hashing}, 
year={2017},}

@article{NSS,
title = "Beyond diffusion process: Neighbor set similarity for fast re-ranking",
journal = "Information Sciences",
volume = "325",
year = "2015",
author = "Xiang Bai and Song Bai and Xinggang Wang",
}

@inproceedings{AnchorGraph,
 author = {Liu, Wei and He, Junfeng and Chang, Shih-Fu},
 title = {Large Graph Construction for Scalable Semi-supervised Learning},
 booktitle = {ICML},
 year = {2010},
} 


@INPROCEEDINGS{ACQ, 
author={G. Irie and H. Arai and Y. Taniguchi}, 
booktitle={ICCV}, 
title={Alternating Co-Quantization for Cross-Modal Hashing}, 
year={2015}, 
}

@inproceedings{MPEC,
  title={An Exact Penalty Method for Binary Optimization Based on {MPEC} Formulation},
  author={Ganzhao Yuan and Bernard Ghanem},
  booktitle={AAAI},
  year={2017}
}

@article{FW,
author = {Frank, Marguerite and Wolfe, Philip},
title = {An algorithm for quadratic programming},
journal = {Naval Research Logistics Quarterly},
volume = {3},
number = {1‐2},
year={1956},
}

@article{FW_convergence,
author = {Lacoste-Julien, Simon},
year = {2016},
month = {07},
title = {Convergence Rate of {F}rank-{W}olfe for Non-Convex Objectives}
}

@inproceedings{ACMR,
 author = {Wang, Bokun and Yang, Yang and Xu, Xing and Hanjalic, Alan and Shen, Heng Tao},
 title = {Adversarial Cross-Modal Retrieval},
 booktitle = {ACM Multimedia},
 year = {2017},
} 

@inproceedings{CVH,
 author = {Kumar, Shaishav and Udupa, Raghavendra},
 title = {Learning Hash Functions for Cross-view Similarity Search},
 booktitle = {IJCAI},
 year = {2011},
} 

@article{CMFH,
  title={Large-Scale Cross-Modality Search via Collective Matrix Factorization Hashing},
  author={Guiguang Ding and Yuchen Guo and Jile Zhou and Yue Gao},
  journal={IEEE TIP},
  year={2016},
  volume={25},
}

@InProceedings{PDH,
  title = 	 {Predictable Dual-View Hashing},
  author = 	 {Mohammad Rastegari and Jonghyun Choi and Shobeir Fakhraei and Daume Hal and Larry Davis},
  booktitle = 	 {ICML},
  year = 	 {2013},
}

@inproceedings{MIRFlickr25k,
 author = {Mark J. Huiskes and Michael S. Lew},
 title = {The {MIR F}lickr Retrieval Evaluation},
 booktitle = {ACM International Conference on Multimedia Information Retrieval},
 year = {2008},
 }

@INPROCEEDINGS{nuswide,
    author = {Tat-seng Chua and Jinhui Tang and Richang Hong and Haojie Li and Zhiping Luo and Yantao Zheng},
    title = {{NUS-WIDE: A} real-world web image database from {N}ational {U}niversity of {S}ingapore},
    booktitle = {CIVR},
    year = {2009}
}

@INPROCEEDINGS{CMDVH,
author={V. E. Liong and J. Lu and Y. Tan and J. Zhou}, 
booktitle={ICCV}, 
title={Cross-Modal Deep Variational Hashing}, 
year={2017}, 
}

@INPROCEEDINGS{DCMH, 
author={Q. Jiang and W. Li}, 
booktitle={CVPR}, 
title={Deep Cross-Modal Hashing}, 
year={2017}, 
month={July},
}

@INPROCEEDINGS{SSAH,
author = {Li, Chao and Deng, Cheng and Li, Ning and Liu, Wei and Gao, Xinbo and Tao, Dacheng},
year = {2018},
booktitle={CVPR}, 
title = {Self-Supervised Adversarial Hashing Networks for Cross-Modal Retrieval}
}

@ARTICLE{SADH, 
author={F. Shen and Y. Xu and L. Liu and Y. Yang and Z. Huang and H. T. Shen}, 
journal={IEEE TPAMI}, 
title={Unsupervised Deep Hashing with Similarity-Adaptive and Discrete Optimization}, 
year={2018}, 
}

@InProceedings{UH-BDNN,
author={Do, Thanh-Toan and Doan, Anh-Dzung and Cheung, Ngai-Man},
title={Learning to Hash with Binary Deep Neural Network},
booktitle={ECCV},
year={2016},
}


@article{ITQ,
  author    = {Yunchao Gong and Svetlana Lazebnik and Albert Gordo and Florent Perronnin},
  title     = {Iterative Quantization: {A} Procrustean Approach to Learning Binary Codes for Large-Scale Image Retrieval},
  journal   = {IEEE TPAMI},
  volume={35}, 
  number={12},
  year      = {2013},
}

@InProceedings{BA,
author = {Carreira-Perpinan, Miguel A. and Raziperchikolaei, Ramin},
title = {Hashing With Binary Autoencoders},
booktitle = {CVPR},
year = {2015}
}

@inproceedings{glove,
  title={Glove: Global vectors for word representation},
  author={Pennington, Jeffrey and Socher, Richard and Manning, Christopher},
  booktitle={EMNLP},
  year={2014}
}



@inproceedings{word2vec,
  title={Efficient estimation of word representations in vector space},
  author={Mikolov, Tomas and Chen, Kai and Corrado, Greg and Dean, Jeffrey},
  booktitle={ICLR Workshop},
  year={2013}
}

@inproceedings{IMH,
 author = {Song, Jingkuan and Yang, Yang and Yang, Yi and Huang, Zi and Shen, Heng Tao},
 title = {Inter-media Hashing for Large-scale Retrieval from Heterogeneous Data Sources},
 booktitle = {ACM SIGMOD},
 year = {2013},
} 

@inproceedings{SpH,
  author    = {Yair Weiss and
               Antonio Torralba and
               Robert Fergus},
  title     = {Spectral Hashing},
  booktitle = {NIPS},
  year      = {2008},
}

@inproceedings{look_imagine_match,
  title={Look, Imagine and Match: Improving Textual-Visual Cross-Modal Retrieval with Generative Models},
  author={Gu, Jiuxiang and Cai, Jianfei and Joty, Shafiq and Niu, Li and Wang, Gang},
  booktitle={CVPR},
  year={2018}
}

@inproceedings{DVSH,
 author = {Cao, Yue and Long, Mingsheng and Wang, Jianmin and Yang, Qiang and Yu, Philip S.},
 title = {Deep Visual-Semantic Hashing for Cross-Modal Retrieval},
 booktitle = {ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
 year = {2016},
} 

@article{VGG,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@inproceedings{LSMVSC,
 author = {Li, Yeqing and Nie, Feiping and Huang, Heng and Huang, Junzhou},
 title = {Large-scale Multi-view Spectral Clustering via Bipartite Graph},
 booktitle = {AAAI},
  year = {2015},
}

@ARTICLE{SSDH, 
author={H. Yang and K. Lin and C. Chen}, 
journal={IEEE TPAMI}, 
title={Supervised Learning of Semantics-Preserving Hash via Deep Convolutional Neural Networks}, 
year={2018}, 
volume={40}, 
number={2}, 
}

@ARTICLE{DH_TIP, 
author={J. Lu and V. E. Liong and J. Zhou}, 
journal={IEEE TIP}, 
title={Deep Hashing for Scalable Image Search}, 
year={2017}, 
volume={26}, 
number={5}, }


@INPROCEEDINGS{SKH, 
author={W. Liu and J. Wang and R. Ji and Y. Jiang and S. Chang}, 
booktitle={CVPR}, 
title={Supervised hashing with kernels}, 
year={2012}, 
}

@ARTICLE{KLSH, 
author={B. Kulis and K. Grauman}, 
journal={IEEE TPAMI}, 
title={Kernelized Locality-Sensitive Hashing}, 
year={2012}, 
}

@book{chung1997spectral,
  title={Spectral graph theory},
  author={Chung, Fan RK and Graham, Fan Chung},
  number={92},
  year={1997},
  publisher={American Mathematical Soc.}
}

@INPROCEEDINGS{AMMSS, 
author={X. Cai and F. Nie and W. Cai and H. Huang}, 
booktitle={ICCV}, 
title={Heterogeneous Image Features Integration via Multi-modal Semi-supervised Learning Model}, 
year={2013}, 
}

@inproceedings{graphHashing,
 author = {Liu, Wei and Wang, Jun and Kumar, Sanjiv and Chang, Shih-Fu},
 title = {Hashing with Graphs},
 booktitle = {ICML},
 year = {2011},
} 

@INPROCEEDINGS{MSRC, 
author={X. Cai and F. Nie and H. Huang and F. Kamangar}, 
booktitle={CVPR}, 
title={Heterogeneous image feature integration via multi-modal spectral clustering}, 
year={2011}, 
}

@article{adagrad,
 author = {Duchi, John and Hazan, Elad and Singer, Yoram},
 title = {Adaptive Subgradient Methods for Online Learning and Stochastic Optimization},
 journal = {J. Mach. Learn. Res.},
 volume = {12},
 year = {2011},
} 

@article{adam,
author = {Kingma, Diederik and Ba, Jimmy},
year = {2014},
title = {Adam: A Method for Stochastic Optimization},
journal = {ICLR}
}

@article{nocedal2006numerical,
  title={Numerical optimization},
  author={Nocedal, Jorge and Wright, Stephen},
  journal={Springer series in operations research, New York, USA},
  year={2006}
}

@incollection{co_reg_MVSC,
title = {Co-regularized Multi-view Spectral Clustering},
author = {Kumar, Abhishek and Rai, Piyush and Hal Daume},
booktitle = {NIPS},
year={2011},
}

@article{CCA,
author = {Hardoon, David R. and Szedmak, Sandor and Shawe-Taylor, John},
title = {Canonical Correlation Analysis: An Overview with Application to Learning Methods},
journal = {Neural Computation},
volume = {16},
number = {12},
year = {2004},
}

@article{cross_retrieval_survey,
  author    = {Kaiye Wang and
               Qiyue Yin and
               Wei Wang and
               Shu Wu and
               Liang Wang},
  title     = {A Comprehensive Survey on Cross-modal Retrieval},
  journal   = {CoRR},
  volume    = {abs/1607.06215},
  year      = {2016},
}

@article{2stephash,
  title={A General Two-Step Approach to Learning-Based Hashing},
  author={Guosheng Lin and Chunhua Shen and David Suter and Anton van den Hengel},
  journal={ICCV},
  year={2013},
}

@inproceedings{SelfTaughtHF,
  title={Self-Taught Hashing for Fast Similarity Search},
  author={Dell Zhang and Jun Wang and Deng Cai and Jinsong Lu},
  booktitle={SIGIR},
  year={2010}
}

@inproceedings{DDCMH,
	author = {Zhen-Duo Chen and Wan-Jin Yu and Chuan-Xiang Li and Liqiang Nie and Xin-Shun Xu},
	title = {Dual Deep Neural Networks Cross-Modal Hashing},
	booktitle = {AAAI},
	year = {2018},
}

@Article{orthogonalProcrustes,
author="Sch{\"o}nemann, Peter H.",
title="A generalized solution of the orthogonal procrustes problem",
journal="Psychometrika",
year="1966",
}

@INPROCEEDINGS{THN,
	author = {Zhangjie Cao and Mingsheng Long and Jianmin Wang and Qiang Yang},
	title = {Transitive Hashing Network for Heterogeneous Multimedia Retrieval},
	booktitle = {AAAI},
	year = {2017},
}

@INPROCEEDINGS{8099765, 
author={D. Mandal and K. N. Chaudhury and S. Biswas}, 
booktitle={CVPR}, 
title={Generalized Semantic Preserving Hashing for N-Label Cross-Modal Retrieval}, 
year={2017}, 
pages={2633-2641}, 
month={July},}

@article{MSAE,
 author = {Wang, Wei and Ooi, Beng Chin and Yang, Xiaoyan and Zhang, Dongxiang and Zhuang, Yueting},
 title = {Effective Multi-modal Retrieval Based on Stacked Auto-encoders},
 journal = {VLDB Endowment},
 issue_date = {April 2014},
 volume = {7},
 number = {8},
 year = {2014},
} 

@ARTICLE{DMHOR, 
author={D. Wang and P. Cui and M. Ou and W. Zhu}, 
journal={IEEE Transactions on Multimedia}, 
title={Learning Compact Hash Codes for Multimodal Representations Using Orthogonal Deep Structure}, 
year={2015}, 
volume={17}, 
number={9}, 
}

@inproceedings{LSSH,
 author = {Zhou, Jile and Ding, Guiguang and Guo, Yuchen},
 title = {Latent Semantic Sparse Hashing for Cross-modal Similarity Search},
 booktitle = {ACM SIGIR},
 year = {2014},
} 

@inproceedings{SAH,
  author    = {Thanh{-}Toan Do and
               Dang{-}Khoa Le Tan and
               Trung T. Pham and
               Ngai{-}Man Cheung},
  title     = {Simultaneous Feature Aggregating and Hashing for Large-scale Image Search},
  booktitle = {CVPR},
  year = {2017},
}

@ARTICLE{DBRC, 
author={D. Hu and F. Nie and X. Li}, 
journal={IEEE Transactions on Multimedia}, 
title={Deep Binary Reconstruction for Cross-modal Hashing}, 
year={2018}, 
}

@INPROCEEDINGS{CMCQ, 
author={T. Zhang and J. Wang}, 
booktitle={CVPR}, 
title={Collaborative Quantization for Cross-Modal Similarity Search}, 
year={2016}, 
}

@inproceedings{CorrAE,
 author = {Feng, Fangxiang and Wang, Xiaojie and Li, Ruifan},
 title = {Cross-modal Retrieval with Correspondence Autoencoder},
 booktitle = {ACM Multimedia},
 year = {2014},
} 

@article{SpectralClusterTutorial,
  title={A tutorial on spectral clustering},
  author={Von Luxburg, Ulrike},
  journal={Statistics and computing},
  volume={17},
  number={4},
  pages={395--416},
  year={2007},
  publisher={Springer}
}

@ARTICLE{SMFH, 
author={J. Tang and K. Wang and L. Shao}, 
journal={IEEE Transactions on Image Processing}, 
title={Supervised Matrix Factorization Hashing for Cross-Modal Retrieval}, 
year={2016}, 
volume={25}, 
number={7}, 
}

@inproceedings{alexnet,
 author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E.},
 title = {ImageNet Classification with Deep Convolutional Neural Networks},
 booktitle = {NIPS},
 year = {2012},
 pages = {1097--1105},
} 

@INPROCEEDINGS{resnet, 
author={Kaiming He and Xiangyu Zhang and Shaoqing Ren and Jian Sun}, 
booktitle={CVPR}, 
title={{Deep Residual Learning for Image Recognition}}, 
year={2016}, 
pages={770--778}
}

@misc{tensorflow,
title={ {TensorFlow}: Large-Scale Machine Learning on Heterogeneous Systems},
url={https://www.tensorflow.org/},
note={Software available from tensorflow.org},
author={
    Mart\'{\i}n~{Abadi}  and others
    },
  year={2015},
}

@misc{tensorpack,
  title={Tensorpack},
  author={Wu, Yuxin and others},
  howpublished={\url{https://github.com/tensorpack/}},
  year={2016}
}

==> [IJCAI20_camera_ready] Network quantization/tex/0_math_def.tex <==
% Mathbf

\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

\newcommand{\hx}{\hat{x}}
\newcommand{\hbW}{\hat{\mathbf{W}}}

\newcommand{\bOnes}{\mathbf{1}}
\newcommand{\bZeros}{\mathbf{0}}

\newcommand{\bTheta}{\mathbf{\Theta}}

\newcommand{\bLm}{\mathbf{L}^m}

\newcommand{\transpose}{\hspace{-0.15em}^\top\hspace{-0.15em}}
\newcommand{\eq}{\hspace{-0.15em}=\hspace{-0.15em}}

% Mathbb
\newcommand{\bbR}{\mathbb{R}}

% Mathcal 
\newcommand{\ndis}{\mathcal{N}}
\newcommand{\xset}{\mathcal{X}}
\newcommand{\oset}{\mathcal{O}}
\newcommand{\vset}{\mathcal{V}}
\newcommand{\tset}{\mathcal{T}}
\newcommand{\uset}{\mathcal{U}}
\newcommand{\dis}{\mathcal{D}}
% \newcommand{\func}{\mathcal{F}}


% other
\newcommand{\func}{\boldsymbol{f}}
\newcommand{\m}{{(m)}}
\newcommand{\mt}{{(t)}}
% \newcommand{\1}{{(1)}}
\newcommand{\M}{{(M)}}

% \newcommand{\(}{\left(}
% \newcommand{\)}{\right)}
% \newcommand{\tanh}{\mathtt{tanh}}
% \newcommand{\sign}{\mathrm{sign}}
% \newcommand{\diag}{\textrm{diag}}
\newcommand{\round}{\mathrm{round}}
% \newcommand{\softmax}{\mathrm{softmax}}


==> [IJCAI20_camera_ready] Network quantization/tex/1_math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\tr}{Tr}
\let\ab\allowbreak




==> [IJCAI20_camera_ready] Network quantization/tex/abstract.tex <==
\begin{abstract}
This paper proposes two novel techniques to train deep convolutional neural networks with low bit-width weights and activations. First, to obtain low bit-width weights, most existing methods obtain the quantized weights by performing  quantization on the full-precision network weights. However, this approach would result in some mismatch: the gradient descent updates full-precision weights, but it does not update the quantized weights. To address this issue, we propose a novel method that enables {direct} updating of quantized weights {with learnable quantization levels} to minimize the cost function using gradient descent. Second, to obtain low bit-width activations, existing works consider all channels equally. However, the activation quantizers could be biased toward a few channels with high-variance. To address this issue, we propose a method to take into account the quantization errors of individual channels. With this approach, we can learn activation quantizers that minimize the quantization errors in the majority of channels. Experimental results demonstrate that our proposed method achieves state-of-the-art performance on the image classification task, using AlexNet, ResNet and MobileNetV2 architectures on CIFAR-100 and ImageNet datasets.


%This paper proposes a novel method to train deep convolutional neural networks with low bit-width weights and activations. To obtain low bit-width weights, most existing methods obtain the quantized weights by performing  quantization on the full-precision network weights. However, this approach could be sub-optimal: the gradient descent updates full-precision weights, but it does not update the quantized weights. To address this issue, we propose a novel method that allows a direct update of quantized weights \red{with learnable quantization levels} to minimize the cost function using gradient descent. To obtain low bit-width activations, existing works consider all channels equally. However, the activation quantizers could be biased toward a few high-variance channels. To address this issue, we propose a method to take into account the quantization errors of individual channels. With this approach, we can learn activation quantizers that minimize the quantization error in the majority of channels. Experimental results demonstrate that our proposed method achieves state-of-the-art performance on the image classification task, using AlexNet and ResNet architectures on CIFAR-100 and ImageNet datasets.
\end{abstract}

==> [IJCAI20_camera_ready] Network quantization/tex/conclusion.tex <==
% \vspace{-3pt}
\section{Conclusion}
% \vspace{-1pt}
In this paper, we have presented a novel method to train CNN with low bit-width weights and activations. Firstly, we proposed to directly learn the quantized weights with learnable quantization levels using gradient descent, instead of learning to quantize full-precision learned weights as proposed in existing works. 
Secondly, by considering the quantization errors of all activation channels, our proposed quantizer for activations  minimizes the information loss in the majority of channels, instead of being biased toward a few high-variance channels.
The experiment results demonstrate the effectiveness of our proposed method in training low bit-width CNN to achieve the competitive classification accuracy for various network architectures.

==> [IJCAI20_camera_ready] Network quantization/tex/exp_analysis.tex <==

%------------------------------------------------------------------------
%------------------------------------------------------------------------

\begin{table*}[ht]
\centering
% \def\arraystretch{1.}
\setlength{\tabcolsep}{8pt}
% \vspace{-7pt}
\begin{threeparttable}
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Methods} &  {Bit-widths}  & \multicolumn{2}{c|}{AlexNet}  &  \multicolumn{2}{c|}{ResNet-18} & \multicolumn{2}{c|}{ResNet-34}  \\ \cline{3-8}
 & {($K_w$/$K_a$)} & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 \\ \hline
 \multicolumn{2}{|l|}{Full-precision (FP)} & 61.8 & 83.5 & 70.3 & 89.5 & 73.8 & 91.4 \\ \hline
 
% BNN  & 1 / 1 & 27.9 & 50.4 & - & - & - & - \\
XNOR-Net  & 1 / 1 & 44.2 & 69.2 & 51.2 & 73.2 & - & - \\ 
% ABC-Net & 1 / 1 & - & - & 42.7 & 67.6 & 52.4 & 76.5 \\ 
Bi-Real Net  & 1 / 1 & - & - & 56.4 & 79.5 & 62.2 & 83.9 \\
% \red{Quantization Networks} & \red{1 / 1} & \red{47.9} & \red{72.5} & \red{53.6} & \red{75.3} & - & -  \\
BONN & 1 / 1 & - & - & {59.3} & \textbf{81.6} & - & - \\
\red{RBCN} & \red{1 / 1} & - & - & \red{\textbf{59.5}} & \red{\textbf{81.6}} & - & - \\
\textbf{LQW + CAQ} & 1 / 1 & \textbf{48.3} & \textbf{72.7} & {56.9} & {79.8} & \textbf{62.4} & \textbf{84.0} \\ \hline
% BENN-SB-6, Boosting$^\ast$  & 1 / 1 & 54.3 & - & 61.0 & - & - & -  \\
% Group-Net (4 bases)$^\ddagger$  & 1 / 1 & - & - & 66.3 & 86.6 & - & -  \\
%   \hline
% BENN-SB-6, Boosting  & 1 / 1 & 54.3 & - & 61.0 & - & - & -  \\

 
DoReFa-Net  & 1 / 2 & 49.8 & - & 53.4 & - & - & - \\ 
% HORQ  & 1 / 2 & - & - & 55.9 & 78.9 & - & -  \\ 
TBN  & 1 / 2 & 49.7 & 74.2 & 55.6 & 79.0 & 58.2 & 81.0 \\
LQ-Nets  & 1 / 2 & 55.7 & 78.8 & 62.6 & {84.3} & \textbf{66.6} & 86.9 \\ 
% Quantization Networks & 1 / 2 & 55.4 & 78.8 & 63.4 & 84.9 & - & - \\
\textbf{LQW + CAQ} & 1 / 2 & \textbf{56.4} & \textbf{79.3} & \textbf{63.1} & \textbf{84.7} & {66.5} & \textbf{87.0} \\\hline
 
DoReFa-Net & 2 / 2 & 48.3 & 71.6 & {57.6} & {80.8} & - & -   \\ 
% PQ + TS + Guided  &  2 / 2 & 52.5 & 77.3 & - & - & - & -  \\
HWGQ  & 2 / 2 & 52.7 & 76.3 & 59.6 & 82.2 & - & -  \\
LQ-Nets  & 2 / 2 & 57.4 & 80.1 & {64.9} & {85.9} & 69.8 & 89.1 \\
DSQ & 2 / 2 & - & - & 65.2 & - & 70.0 & - \\
QIL  & 2 / 2 & \textbf{58.1} &  - & 65.7 & - & \textbf{70.6} & - \\
\textbf{LQW + CAQ} &  2 / 2 & {57.8} & \textbf{80.4} & \textbf{66.0} & \textbf{86.2} & {70.5} & \textbf{89.4}  \\ \hline
Group-Net  & 4 bases$^\ddagger$ & - & - & 66.3 & 86.6 & - & -  \\
  \hline
 
\end{tabular}
\begin{tablenotes}
\footnotesize
% \item\hspace{-1em}  $^\dag$ The results for AlexNet with $K_w$/$K_a=2/2$ are quoted from \cite{guidedQuantize}. 
% For DoReFa-Net using ResNet-18 with $K_w$/$K_a=2/2$, we use the official released code to evaluate.
% (\url{https://github.com/tensorpack/tensorpack/tree/master/examples/DoReFa-Net}).
\item $^\ddagger$ The complexity of 4-base Group-Net for a convolution is comparable to ours at $K_w$/$K_a=2/2$.
\item ``-'' indicates that the results are not provided.
\end{tablenotes}
\end{threeparttable}
\vspace{-5pt}
\caption{Top-1/Top-5 classification accuracy (\%) of AlexNet and ResNet-18/34 on ImageNet dataset under different bit-widths.  }
\label{tab:compare_imagenet}
\vspace{-9pt}
\end{table*}



% \vspace{-3pt}
\subsection{Ablation Analysis}
% \vspace{-2pt}
In this section, we first conduct experiments to analyze the effect of our proposals, i.e., \textbf{\textit{(i)}} directly learning the quantized weights (LQW) and \textbf{\textit{(ii)}} the channel-wise average quantizer (CAQ) for activations. For easy comparison, we consider the learned quantizer proposed by \citeauthor{LQNets}, which is used for both weights and activations, as the baseline. Table \ref{tb:ablation_study} shows the classification accuracy of AlexNet on CIFAR-100 with different combinations of baseline method and our proposals for $K_w/K_a\hspace{-1pt}=\hspace{-1pt}2/2$. 
% In this experiment, we use the setting of 2-bit quantization for both weights and activations ($K_w/K_a=2/2$). 
The experimental results demonstrate the effectiveness of our proposals, i.e., LQW and CAQ, in training networks with low bit-width weights and activations. Additionally, LQW helps achieve a slightly higher improvement gain compared to CAQ ($+0.1\%$).


We additionally conduct an experiment on CIFAR-100 using AlexNet with different numbers of CAQ iteration $T$. We repeat the experiment 5 times and report the results (mean$\pm$std) in Table \ref{tab:num_iter}. We observer that using $T = 2,3$ does not result in any significant difference on Top-1 accuracy compared to $T = 1$. 
This is mainly because, for each mini-batch, CAQ starts from proper initial quantization basis values, which are the good results of the last mini-batch.

==> [IJCAI20_camera_ready] Network quantization/tex/exp_compare_sota.tex <==




% \vspace{-2pt}
\subsection{Comparison With State of The Art}
% \vspace{-1pt}
In this section, we compare the performance of our proposed method with
existing methods including 
% BNN \cite{BNN}, 
XNOR-Net \cite{xnor_net}, DoReFa-Net \cite{dorefa}, 
%ABC-Net \cite{NIPS2017_6638}, HORQ \cite{HORQ}, 
HWQG \cite{hwgq}, PQ+TS+Guided \cite{guidedQuantize},
TBN \cite{tbn}, LQ-Nets \cite{LQNets}, Bi-Real Net \cite{bi-real}, QIL \cite{QIL},
%BENN \cite{binary_ensemble_NN},  PCNN \cite{pcnn}, %
DSQ \cite{dsq}, BONN \cite{bonn}, RCBN \cite{RBCN}, 
% Quantization Networks \cite{Yang_2019_CVPR},
and Group-Net \cite{groupnet}. 
% \red{Noting that, although our method is generic and can be used with any bit-width, architecture; in the experiments, we mainly focus on very low bit-widths, e.g., 1 or 2 bits, and AlexNet, ResNet, and MobileNetV2 architectures.}
Noting that, our method is generic and can be used with any bit-width and architecture.
%e.g., AlexNet, ResNet, and MobileNetV2.


% \textbf{Comparison on CIFAR-100.} 
\paragraph{Comparison on CIFAR-100.}
Table \ref{tb:compared_cifar100} presents the top-1/top-5 classification accuracy on CIFAR-100 dataset of different network quantization methods on AlexNet, ResNet-18, and MobileNetV2. In all compared settings for AlexNet and ResNet-18, our method consistently outperforms the state-of-the-art method LQ-Nets by large margins, i.e., $\ge 0.7\%$ for $K_w/K_a=1/2$ and $\ge 0.6\%$ for $K_w/K_a=2/2$ in term of top-1 accuracy. 
\red{Regarding the efficient architectures MobileNetV2, at bit-widths of $K_w/K_a=3/3$, there is only a small accuracy drop compared with FP model.
Even at lower bit-width $K_w/K_a=2/2$, $K_w/K_a=1/2$, our proposed method still achieves good performance for MobileNetV2, which is already very efficient. This confirms the effectiveness of our proposed method.}
Furthermore, we can observe from Figure \ref{fig:cross_entropy_loss} that the training loss on CIFAR-100 of LQ-Nets with ResNet-18 architecture is unable to approach $0$ as our proposed method does. LQ-Nets also suffers from unstable test error (Figure \ref{fig:test_error}).
This result is potentially due to the mismatch in the training process of LQ-Nets, as the gradient descent does not directly update the quantized weights. Consequently, the quantized weights are unable to obtain the desirable changes.
This demonstrates the necessity of direct updating the quantized weights using gradients as our proposed method can do.




% \vspace{-1pt}
% \textbf{Comparison on ImageNet.}
\paragraph{Comparison on ImageNet.}
The classification results on ImageNet dataset for AlexNet and ResNet-18/34 are presented in Table \ref{tab:compare_imagenet}. 
% In this experiment, we only focus on the very low bit-width setting, e.g., 1 or 2 bits for weights and 2 bits for activation. 
Our proposed method (LQW + CAQ) outperforms the compared methods, e.g., DoReFa-Net, TBN, HORQ, HWGQ, DSQ, in the majority of settings for both AlexNet and ResNet-18/34. 
% For $K_w/K_a=1/2$, the absolute improvement of top-1 accuracy of our method over the most competitive one, LQ-Nets \cite{LQNets}, is $+0.4\%$ for AlexNet and $+0.3\%$ for ResNet-18. For $K_w/K_a=2/2$, we outperforms LQ-Nets by $+0.6\%$ top-1 accuracy for AlexNet, while achieving comparable performance on ResNet-18 ($+0.1\%$ top-1 accuracy improvement).
Our method outperforms LQ-Nets in term of Top-1 accuracy by clear margins in the majority of experiments (i.e., $\ge 0.4\%$);
except for ResNet-34 with $K_w/K_a = 1/2$, where our method achieves comparable performance with LQ-Nets.
% ($0.1\%$ lower for Top-1 and $0.1\%$ higher for Top-5).
For $K_w/K_a = 1/1$, our method gains 0.5\% and 0.2\% Top-1 improvement over Bi-Real Net for ResNet-18 and ResNet-34 respectively. Our method still under-performs BONN \red{and RBCN} for ResNet-18. However, BONN is designed specifically for 1-bit CNN, it is nontrivial to adopt this method to higher bit-widths for better trade-off between the computational speed and accuracy, as can be done easily in our proposed method. \red{Besides, in BONN, in addition to quantization loss and the essential cross-entropy loss, BONN also has an additional feature loss %(i.e., center loss) 
to enhance the intra-class compactness which improves the classification accuracy. For our work, because we aimed to learn the quantized network without any modification in the network architecture, in addition to cross-entropy, we only introduce the quantization loss. 
%We note that, in principle, the feature loss in BONN can be integrated in our method to improve the classification accuracy. 
{Regarding RBCN, this method requires joint training of a FP model, a quantized model, and discriminators for distillation from the FP model to the a quantized model. Consequently, this method requires significantly high computational cost and memory.}}
In comparison to QIL, our method achieves comparable performance for $K_w/K_a=2/2$. Specifically, our method has 0.3\% Top-1 accuracy lower than QIL for AlexNet, while achieves 0.3\% higher than QIL for ResNet-18. For ResNet-34, the accuracy of our method is marginally lower than QIL's (i.e., -0.1\% top-1 accuracy). We note that QIL usually achieves the best performance with trainable but complex quantizer functions. It is unsure if the computational complexity of QIL during inference can be linearly proportional to the bit-widths of weights and activations (no efficiency analysis is provided by \citeauthor{QIL}). In our work, we carefully design the method to 
% maximize the capability of quantizers while 
ensure the complexity linearly proportional to the bit-widths. 
Additionally, in comparison with Group-Net (4 bases) on ResNet-18, our method has 0.3\% lower in top-1 accuracy.
Nevertheless, Group-Net requires additional computational costs for the skip-connection in every binary convolution 
%with complexity of $\mathcal{O}(KN_a)$ 
and for computing the soft connection between binary groups.
% with complexity of $\mathcal{O}(KN_a)$, where $N_a$ is the number of output elements of a particular binary conv./group.
% \footnote{Since the implementation using bitwise operation of Group-Net is not provided, actually running time comparison between our method and Group-Net is not possible.}.


==> [IJCAI20_camera_ready] Network quantization/tex/exp_efficiency_analysis.tex <==
\begin{figure*}[]
\centering
% \vspace{-10pt}

\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth]{fig/speedup_cpp.pdf}
\caption{1 thread w/o SIMD}
\label{fig:speedup_cpp}
\end{subfigure}
$\qquad$
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth]{fig/speedup_simd.pdf}
\caption{1 thread with SIMD}
\label{fig:speedup_simd}
\end{subfigure}
$\qquad$
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth]{fig/speedup_blas.pdf}
\caption{CBLAS (8 threads)}
\label{fig:speedup_blas}
\end{subfigure}
\vspace{-5pt}
\caption{The speedup of one convolution by varying input channel size at different bit-widths.}
\label{fig:speedup}
\vspace{-9pt}
\end{figure*}


% \vspace{-2pt}
\subsection{Inference Efficiency Analysis}
\label{sec:efficicency_analysis}
% \vspace{-1pt}
% \subsubsection{Inference:}~ 
We first show that the inner products between our quantized weight and activation vectors can be efficiently computed by bitwise operations. Let a weight vector $\bW \in \bbR^N$ be encoded by $\bS^{w}=\{\bs_1^{w},\cdots,\bs_{K_w}^{w}\} \in \{-1, 1\}^{N\times K_w}$ and the learned basis vector $\bv^w=\{v_1^w,\cdots, v_{K_w}^w\} \in \bbR^{K_w}$.
Similarly, we encode an activation vector $\bA \in \bbR^N$ by $\bS^{a}=\{\bs_1^{a},\cdots,\bs_{K_a}^{a}\}\in \{0, 1\}^{N\times K_a}$ and $\bv^a=\{v^a_1,\cdots,v^a_{{K_a}}\}$ $\in \bbR^{{K_a}}$.
To utilize the bitwise inner products \cite{dorefa}; first we need to convert $\bS^{a}\in \{0, 1\}^{N\times K_a}$ to $\hat{\bS}^{a}\in\{-1,1\}^{N\times K_a}$ by $\bS_i^{a} = 0.5\hat{\bS}_i^{a} +0.5$.
Then, with some manipulation, we can derive that:
% \vspace{-5pt}
\begin{equation}
\label{eq:bitwise_dot_product}
\hspace{-5pt}\mathcal{Q}(\bW,\bv^w)^\top\mathcal{Q}(\bA, \bv^a)=Q+\hspace{-2pt} \sum_{i=1}^{K_w}\sum_{j=1}^{{K_a}}\frac{v_i^wv_j^a}{2}\left(\bs_i^{w}\odot\hat{\bs}_j^{a}\right),
% \vspace{-3pt}
\end{equation}
where $Q = \sum_{i=1}^{K_w}\sum_{j=1}^{{K_a}}\frac{v_i^wv_j^a}{2}\left(\bs_i^{w}\odot \boldsymbol{1}\right)$, $\boldsymbol{1}$ is a $K_a$-dimension vector with all elements are 1, and $\odot$ denotes the inner product with bitwise operations, \textit{xnor} and \textit{popcnt}. Noting that during inference, $\bS^w$, $\bv^w$, and $\bv^a$ are fixed; so $Q$ is a scalar constant and can be pre-computed. Similar to \cite{dorefa,LQNets}, the computation complexity of Eq. \ref{eq:bitwise_dot_product} w.r.t. $K_w,K_a$ is $\mathcal{O}(K_w{K_a})$, i.e., directly linear-proportional to the bitwidths of weights and activations. 

Considering a matrix multiplication (MatMul) $\widetilde{\bC}=\widetilde{\bW}\widetilde{\bA}$, where $\widetilde{\bW}\in \bbR^{n\times p}$, $\widetilde{\bA}\in \bbR^{p\times m}$ and  $\widetilde{\bC}\in \bbR^{n\times m}$. 
To calculate $\widetilde{\bC}$ with FP $\widetilde{\bW}, \widetilde{\bA}$, there are $n m q$ multiply-accumulate operations (MACs) required.
Following \citeauthor{tbn}, the theoretical speedup ratio for the bitwise MatMul of our method, which requires $K_w{K_a} mn$ MACs and $2(K_w{K_a})mn$ binary operations, is given as follows:
\begin{equation}
\label{eq:speedup}
S = \frac{\gamma q}{\gamma K_w{K_a}+2(K_w{K_a})\lceil\frac{q}{L}\rceil},
\end{equation}
where $L$ is the number of bits binary operation in one clock cycle, and  $\gamma = 1.91$ is ratio between the speed of performing a $L$-bit binary operation and a MAC \cite{tbn}. 


However, we found that Eq. \ref{eq:speedup} may not accurately reflect the actual speedup ratio of MatMul using bitwise operations in comparison with using FP.
First, Eq. \ref{eq:speedup} over-simplifies the bitwise MatMul by only including \textit{xnor} and \textit{popcount} operations. In fact, additional operations are required, including \textit{sum} to accumulate the \textit{popcount} results, operations to convert from integer (\textit{popcount} results) to FP numbers to multiply with quantization basis values. 
Second, Eq. \ref{eq:speedup} under-utilizes the CPU capability with FP computation. The modern CPU can perform 4 MACs in a single clock by using Single Instruction Multiple Data (SIMD) instructions. Multi-threading can also be utilized to further speed up computation by dividing the workload into multiple separate cores.   
Third, data transferring operations (e.g., loading, storing) is not considered. 
Using quantized weights and activations or SIMD can help to reduce the number of loading/storing operations. 
Finally, the additional time for quantizing activations should be considered in computing the speedup ratio.


We provide a CPU implementation of the bitwise MatMul (Eq. \ref{eq:bitwise_dot_product}) to measure its actual CPU speedup in comparison with FP MatMul. We fix $n=256$ (i.e., the number of output channels $C_o$), $m=14 \times  14 \times  100$ (i.e., an 100-sample mini-batch of $14 \times  14$ size), and $3 \times 3$ kernel. Noting that $p=3\times 3\times C_i$, where $C_i$ is the number of input channels.
% ~\footnote{Most common kernel size.}. 
The experiment is conducted on a quad-core CPU (i7-6700HQ@2.60GHz) with $L=64$. In Figure \ref{fig:speedup}, we present the empirical speedup ratio of the bitwise MatMul in compared with the FP MatMul (with different implementations of FP MatMul) as the number of input channels $C_i$ varies. 


Firstly, from Eq. \ref{eq:speedup}, we can compute the theoretical speedup for $K_w/K_a=1/1$ is $\sim\hspace{-2pt}60\times$. However, our CPU implementation of bitwise MatMul, with all overheads including quantization and memory allocation, can achieve up to $\sim\hspace{-2pt}200\times$ speedup (Figure \ref{fig:speedup_cpp}) (when SIMD is not utilized for FP MatMul). 
% This speedup ratio is $\sim 3.3$ times higher the theoretical speedup. 
When SIMD is utilized for FP MatMul, bitwise MatMul can achieve about $\sim\hspace{-2pt}23\times$ speedup for $K_w/K_a=1/1$ (Figure \ref{fig:speedup_simd}).
Additionally, when multi-threading (8 threads) is also considered for both FP (CBLAS library)
% \footnote{We use the highly-optimized CBLAS library.} 
and bitwise MatMul, bitwise MatMul can gain $\sim\hspace{-2pt} 4.3\times$ speedup for $K_w/K_a=1/1$. While for $K_w/K_a=2/2$, we obverse only a small speedup for bitwise MatMul (for $C_i>64$) (Figure \ref{fig:speedup_blas}).
Furthermore, the empirical speedup ratios confirm that the complexity of our bitwise MatMul is proportional to the bit-widths of weights and activations.

\red{Additionally, we presented in Table \ref{tb:reference_time} the inference time per image using bitwise convolution for the quantized AlexNet (for both weight and activation) models. We also include the inference time using FP convolution operation for comparison. We can see that when using AlexNet with ${K_w}/{K_a}=1/2$, our proposed method with bitwise convolution can speed up $\times$1.7 and $\times$6.8 in comparison with FP convolution with and without using SIMD, respectively.}


%==================================================================
\begin{table}[]
\setlength{\tabcolsep}{8pt}
\centering
% \vspace{-5pt}
% \def\arraystretch{1.05}
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{FP} & \multicolumn{2}{c|}{Bitwise} \\ \hline
W/o SIMD & With SIMD & 2 / 2 & 1 / 2 \\ \hline
3254$\pm$28 & 809$\pm$19 & 523$\pm$5 & 475$\pm$8 \\\hline
% ResNet18 & & & & \\\hline
\end{tabular}
\vspace{-4pt}
\caption{The average $\pm$ std of inference time (ms) for 1 image using AlexNet trained on CIFAR-100 dataset under FP and bit-wise conv. implementations. 
The experiments was conducted on a CPU(i7-6700HQ@2.60GHz) with single-thread using 10 random images.
}
\label{tb:reference_time}
\vspace{-7pt}
\end{table}

%==================================================================
\begin{table}[t]
% \def\arraystretch{1.05}
\setlength{\tabcolsep}{8pt}
\centering
\begin{tabular}{|c|c|c|}
\hline
Weight & Activation & Top-1  \\\hline
Baseline & Baseline & 69.2 \\
Baseline & \textbf{CAQ} & 69.6 \\
\textbf{LQW} & Baseline  & 69.7 \\
\textbf{LQW} & \textbf{CAQ} & 69.9 \\\hline
\end{tabular}
\vspace{-5pt}
\caption[Top-1 accuracy  (\%) of AlexNet on CIFAR-100 dataset using different methods (LQW, CAQ, and baseline) with $K_w/K_a=2/2$.]
{Top-1 accuracy  (\%) of AlexNet on CIFAR-100 dataset using different methods (LQW, CAQ, and baseline \cite{LQNets}) with $K_w/K_a=2/2$.}
\label{tb:ablation_study}
\vspace{-5pt}
\end{table}

%====================================================================
% \vspace{-15pt}
\begin{table}[t]
\centering
% \small
% \def\arraystretch{1.05}
\setlength{\tabcolsep}{6pt}
% \vspace{-6pt}
\begin{tabular}{|c|c|c|c|}
\hline
{Bit-widths} & \multicolumn{3}{c|}{Top-1 Accuracy (\% - mean$\pm$std)} \\ \cline{2-4}
{($K^w$/$K^a$)}  &  $T=1$ & $T=2$ & $T=3$ \\ \hline
1 / 2 & 69.42$\pm$0.14 & 69.59$\pm$0.16 & 69.55$\pm$0.12  \\
2 / 2 & 69.88$\pm$0.11 & 70.03$\pm$0.13 & 69.82$\pm$0.09 \\
\hline
\end{tabular}
\vspace{-5pt}
\caption{Accuracy w.r.t. numbers of CAQ iteration $T$}
\label{tab:num_iter}
\vspace{-8pt}
\end{table}
%====================================================================



%=====================================================================
\begin{table*}[t]
\centering
% \def\arraystretch{1.05}
\setlength{\tabcolsep}{7.5pt}
% \vspace{-5pt}
\begin{threeparttable}
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Methods} & {Bit-widths}  & \multicolumn{2}{c|}{AlexNet}  & \multicolumn{2}{c|}{ResNet-18} & \multicolumn{2}{c|}{ \red{MobileNetV2}}  \\ \cline{3-8}
 &  {$({K_w}/{K_a})$} & Top-1 & Top-5 & Top-1 & Top-5 & \red{Top-1} & \red{Top-5} \\ \hline
\multicolumn{2}{|l|}{Full-precision (FP)} & 71.2 & 91.3 & 74.0 & 92.7 & \red{72.9} & \red{92.1} \\ \hline
%\multicolumn{2}{|c|}{Full-precision} & 71.2 & 91.3 & 74.0 & 92.7 \\ \hline

% PQ+TS+Guided & 4 / 4 & 65.8 & 88.6 & - & - \\
% DoReFa-Net$^\dag$  & 4 / 4 & 64.9 & 88.5 & 67.7 & 90.2 \\  \hline
LQ-Nets  & 3 / 3 & 70.9 & 91.3 & 72.9 & 92.2 & - & -  \\
\textbf{LQW + CAQ} & 3 / 3  & \textbf{71.3} & \textbf{91.3}  & \textbf{73.0} & \textbf{92.3} & \red{\textbf{71.5}} & \red{\textbf{91.6}} \\ \hline
 
PQ+TS+Guided & 2 / 2 & 64.6 & 87.8 & - & - & - & - \\
DoReFa-Net  & 2 / 2 & 63.4 & 87.5 & 65.1 & 88.0 & \red{56.8} & \red{85.2} \\ 
LQ-Nets & 2 / 2 & 69.2 & 91.2 & 70.8 & 91.3 & - & - \\
\textbf{LQW + CAQ} & 2 / 2  & \textbf{69.9} & \textbf{91.3} & \textbf{72.1} & \textbf{92.3} & \red{\textbf{65.5}} & \red{\textbf{89.6}} \\ \hline
 
LQ-Nets & 1 / 2 & 68.7 & 90.5 & 70.4 & 91.2 & - & - \\
\textbf{LQW + CAQ}  & 1 / 2  & \textbf{69.3} & \textbf{91.2} & \textbf{72.1} & \textbf{91.6} & \red{\textbf{63.0}} & \red{\textbf{88.27}} \\ \hline
 
\end{tabular}
\begin{tablenotes}
\footnotesize
% \item $^\dag$ The results are quoted from \cite{guidedQuantize} for AlexNet.
\item ``-'' indicates that the results are not provided.
\end{tablenotes}
\end{threeparttable}
\vspace{-6pt}
\caption{Top-1/Top-5 accuracy (\%) of AlexNet, ResNet-18, \red{and MobileNetV2} on CIFAR-100 dataset under different bit-widths. }
\label{tb:compared_cifar100}
\vspace{-4pt}
\end{table*}
%=====================================================================


%===================================================================
\begin{figure}[t]
% \vspace{-4pt}
\centering
% \captionof{figure}{The cross-entropy loss (a) and test error (b) ResNet-18 on CIFAR-100 dataset with $K_w/K_a=1/2$.}
% \vspace{-5pt}
\begin{subfigure}[b]{0.235\textwidth}
\includegraphics[width=\textwidth]{fig/loss_resnet_cifar100.png}
\caption{Cross-entropy loss}
\label{fig:cross_entropy_loss}
\end{subfigure}
% $\qquad$
\begin{subfigure}[b]{0.235\textwidth}
\includegraphics[width=\textwidth]{fig/error_resnet_cifar100.png}
\caption{Test error}
\label{fig:test_error}
\end{subfigure}
\vspace{-5pt}
\caption{The cross-entropy loss (a) and test error (b) ResNet-18 on CIFAR-100 dataset with $K_w/K_a=1/2$.}
\label{fig:classification_error}
\vspace{-10pt}
\end{figure}




==> [IJCAI20_camera_ready] Network quantization/tex/experiments.tex <==
\vspace{-3.5pt}
\section{Experiments}
\vspace{-1pt}
To evaluate the performance of the proposed methods, we conduct experiments on CIFAR-100 \cite{cifar10} and ImageNet (ILSVRC2012) \cite{imagenet} datasets using the two representative network architectures, AlexNet \cite{alexnet}, ResNet \cite{resnet}, and \red{MobileNetV2 \cite{MobileNetV2}}. We adopt the standard data splits for both datasets, i.e., 50K training and 10K test images for CIFAR-100, about 1.2 million training and 50K test images for ImageNet.
Additionally, we use a variant of AlexNet architecture by adding Batch Normalization layers after each convolutional layer and Fully-Connected layer and removing the Local Response layers as \red{commonly used in recent works \cite{dorefa,guidedQuantize}.} 

\vspace{-3pt}
\subsection{Implementation Details}
We follow the common settings in previous works \cite{dorefa,LQNets}: We first resize the shorter side of the images to $256$. During training, we randomly crop  $227\times 227$/$224\times 224$ patches for AlexNet/ResNet and MobileNetV2 from training images or their horizontal flips (called as basic augmentation). Following \citeauthor{LQNets}, we adopt the basic augmentation in most of our experiments, except for the cases of ResNet on ImageNet dataset with $K_w/K_a=2/2,3/3$, where the augmentation strategy of the ResNet Torch implementation\footnote{\url{https://github.com/facebook/fb.resnet.torch}} is adopted. We report top-1 and top-5 classification accuracy using single-center crops of test images. 
% For CIFAR-100, we conduct experiments 5 times and report the average accuracy.

% \vspace{-2pt}
In all experiments, we use Nesterov SGD with a momentum of $0.9$ and  mini-batch size of $256$. The starting learning rate is set at $0.02 / 0.1/0.02$ for AlexNet/ResNet\red{/MobileNetV2} respectively. We adopt the polynomial learning rate scheduler with the annealing power of 2 and the final learning rate of $10^{-6}$ after $120$ epochs. Regarding the weight decay, for FP weights, we set weight decay as $5 \times  10^{-4}$/$5 \times  10^{-5}$/$10^{-5}$ for AlexNet/ResNet\red{/MobileNetV2}. For the quantized weights, the weight decay has a stronger effect; hence, we cross-validate within $\{10^{-6},5 \times  10^{-6},$ $ 10^{-5}, 5 \times  10^{-5}\}$ using 1\% of the training set as the validation set.
We scale the learning rate of the binary weight encodings as suggested by \citeauthor{BinaryConnect}. 
% However, instead of using the initialization coefficients from \cite{xavier_init}, we empirically found that a scaling factor of $\gamma_\bs=50$ work well in general. 
We also scale the learning rate of quantization basis vectors by a factor of $\gamma_\bv=\frac{1}{50}$ to avoid unstable training. The moving-average factor $\mu$ and the number of iteration $T$ in CAQ algorithm are fixed as $0.9$ and $1$, respectively.
%
Following previous works \cite{xnor_net,dorefa,LQNets}, we do not quantize the first and last layers. Since the speedup, benefited by bitwise operations, is low due to their small input-channel number or filter size \cite{dorefa,xnor_net}.   
% Additionally, to maximize the flexibility of the low bit-width DNN while still ensure its compatibility with bitwise operations, we learn one quantizer per activation layer and one quantization level vector per filter.
% The quantization basis vectors for quantized weights/activations are initialized using uniform quantization.
All networks using our proposed method are trained from scratch.  
% Our proposed method is implemented with TensorFlow %\cite{tensorflow} 
% and trained with the aid of Tensorpack.
%\cite{tensorpack}.

\input{tex/exp_efficiency_analysis.tex}
\input{tex/exp_analysis.tex}
\input{tex/exp_compare_sota.tex}



% 



==> [IJCAI20_camera_ready] Network quantization/tex/introduction.tex <==
% \vspace{-3pt}
\section{Introduction}
Deep Convolutional Neural Networks (CNNs) have been playing a crucial role in the recent tremendous successes of a variety of computer vision tasks including image classification, object detection, segmentation, image retrieval, to name a few. However, unfortunately, this benefit comes at the cost of an excessive amount of memory and expensive computational resources, which impedes its application in embedded devices. 
% For instance, the ResNet-152 \cite{resnet} model requires up to $11.3$ billion FLOPs to classify a single $224 \times 224$ image and consumes about 230MB storage for the model. 
Therefore, how to make CNN lightweight and practical in terms of memory and computation is an important task and has attracted a great amount of effort.

An effective approach is to use low bit-width weights and/or low bit-width activations. This approach not only can reduce the memory footprint, but it also achieves a significant gain in speed. In particular, using binary weights with full-precision (FP) activations can reduce the model size by $32 \times$ and achieve $\sim\hspace{-3pt}2\times$ faster during inference \cite{xnor_net}. When also using low bit-width activations, the speedup is significantly greater; as the most computationally expensive convolutions can be done by bitwise operations \cite{xnor_net}.
Even though there are great improvements achieved by the existing quantization-based methods \cite{hwgq,lossaware,HORQ,xnor_net,tbn,LQNets,dorefa,TTQ}, there are still noticeable accuracy gaps between the quantized CNNs and their FP counterparts, especially in the challenging cases of 1 or 2 bit-width weights and activations. 

%Most of the current state-of-the-art network quantization methods \cite{TWN,tbn,LQNets,dorefa,TTQ} learn the FP weights and their corresponding quantizers either in advance (i.e., quantize a pretrained FP weight) or jointly (i.e., learn the FP weights and their quantizers simultaneously).
Most of the current state-of-the-art network quantization methods \cite{tbn,LQNets,dorefa,TTQ,zhou:2018} learn the FP weights and the quantizers to quantize FP weights. The learning can be sequential or joint learning. In the sequential learning, the models firstly learn FP weights. They then learn the quantizers to quantize FP weights. In the joint learning, the models learn the FP weights and their quantizers simultaneously. 
However, both learning approaches cause mismatch during training, i.e., the gradient descent process is only used to update the FP weights, but not the quantized weights.
To address this problem, we propose a novel method that allows gradients to update the quantized weights with learnable quantization levels directly, i.e., the quantized weights are learned without requiring FP weights. In specific, the quantized weights are learned via learning two auxiliary variables: binary weight encodings and quantization basis vectors.
%Furthermore, our proposed method to directly learn the quantized weights can be considered as a generalized version of Binarized Neural Networks \cite{BinarizedNN}.  

Another important aspect of training a low bit-width network is the activation quantization. Earlier works use simple, hand-crafted quantizers (e.g., uniform or logarithmic quantization) \cite{DL_limited_num_precision,fix_point_quant,dorefa,INQ,QNN} or pre-computed quantizers fixed during network training \cite{hwgq}. Recently, \cite{LQNets,QIL} proposed to learn the quantizers for activations during training adaptively. 
However, all existing methods consider all activation channels of an activation map 
equally and do not pay attention to the fact that different channels of activations contain different amount of information.
% (i.e., different channels have different variances).
As a result, the learned quantizer could be biased toward a few channels with high variances; while losing information from a large number of lower-variance channels.
To handle this problem, we propose a novel activation quantization method which tries to minimize the information loss in the majority of channels, which cumulatively have noticeable impacts on outputs, via learning channel-wise quantizers (i.e., one quantizer per channel). 
% Furthermore, we found that the theoretical speedup used in a recent work \cite{tbn} has several problems and does not reflect the true speedup ratio of matrix multiplication using bitwise operations in comparison with using FP\footnote{More details will be discussed in section \ref{sec:efficicency_analysis}.}. Hence, to obtain more accurate speedup ratio, we provide a CPU implementation of the bitwise matrix multiplication.
Our main contributions can be summarized as follows:

\begin{itemize}[leftmargin=10pt]
\item % Firstly, our work is the first one to propose a novel method to learn the quantized weights directly, instead of learning to quantize the full precision weights. Our proposed method allows the quantized weights to be updated using gradient descent such that they directly minimize the cost function. Hence, our method could avoid the training mismatch (i.e., the quantized weights are not updated by gradients) of existing methods.
% This avoids the mismatch training issue of existing methods
Our work is the first one to propose a novel method to learn the quantized weights \red{with learnable quantization levels} directly by using gradient descent such that they directly minimize the cost function. Hence, our method could avoid the training mismatch (i.e., the quantized weights are not updated by gradients) of existing methods.
% This avoids the mismatch training issue of existing methods
\item To avoid the activation quantizers being biased toward a few high variance activation channels, we propose to learn quantizers that focus  %on quantization levels that 
to minimize quantization errors of the majority of channels. 
This is obtained via learning channel-wise quantizers. 
%The quantizers are obtained by considering channel-wise quantization errors when computing the layer-wise quantizers.
% firstly consider the quantization error of each channel of activation independently, i.e., learning channel-wise quantizers. Then, the layer-wise quantizer  
% \item Thirdly, we provide CPU implementation of the matrix multiplication using bitwise operations to provide more accurate speedup ratio. 
\item A detailed analysis on the  inference efficiency of the proposed method is provided. The proposed method also achieves the state-of-the-art image classification accuracy when comparing to other low bit-width networks on CIFAR-100 and ImageNet datasets with AlexNet, ResNet and MobileNetV2 architectures. 
%experimental results show that the proposed method achieves the state-of-the-art image classification accuracy for low bit-width networks 
%on CIFAR-100 and ImageNet datasets with AlexNet and ResNet architectures.
% on the CIFAR-100 \cite{cifar10} and ImageNet \cite{imagenet} datasets with AlexNet \cite{alexnet} and ResNet \cite{resnet} architectures.
\end{itemize}


==> [IJCAI20_camera_ready] Network quantization/tex/proposed_method.tex <==
% \vspace{-3pt}
\section{Proposed Method}



% \vspace{-2pt}
\subsection{Learned Quantized Weights}
Apart from existing network quantization works, which train the weight quantizers from the full-precision (FP) network weights either jointly or in advance \cite{dorefa,tbn,LQNets}; in this work, we propose to directly learn the quantized weights. 
% Specifically, for a general case of representing a network weight $\bW_q$ of $N_w$ elements by $K_w$-bits, we learn a binary weight encoding $\bS^w\in\{-1,+1\}^{N_w\times K_w}$ and a quantization basis vector $\bv^w=[v_1^w,\cdots, v_{K_w}^w]\in\bbR^{K_w}$. Consequently, the network weight can be directly replaced by $\bS^w\bv^w$ in the cost function, i.e., $\bW_q=\bS^w\bv^w$.
% \begin{equation}
%     \min_{\Theta}\mathcal{L}(\Theta),\quad \textrm{s.t. } \bS_i^w\in\{-1,+1\}^{N_w\times K_w} ~~\forall i,
% \end{equation}
% where $\Theta=\{\bS_i^w,\bv_i^w\}_{\forall i}$ is the set of all network parameters and $\mathcal{L}$ is a cost function, e.g., cross-entropy for classification task. Note that, to maximize the flexibility of the low bit-width CNN, while ensuring its compatibility with bitwise operations, we learn one quantization basis vector and weight encoding per filter.

% To handle the binary constraint on the weight encoding $\bS^w$, inspired by \cite{BinaryConnect}, we only binarize $\bS^w$  during the forward (i.e., using $\sign$ function) and backward propagations, and keep $\bS^w$ in full-precision values (i.e., $\bS^w\in\bbR^{N_w\times K_w}$) for parameter updates. Furthermore, in order to update $\bS^w$ using gradient descent, we adopt the straight-through estimator (STE) \cite{STE}, i.e., ${\partial\sign(z)}/{\partial z}=1_{|z|\le 1}$, to approximate the gradients propagating through the $\sign$ function. 
% Regarding the quantization basis vectors $\bv^w$, as they have no constraint, they can be updated normally using the standard gradient descent process.
% The proposed method allows the quantized weights to be updated (via the weight encodings and the quantization basis vectors) such that they directly minimize the final cost function through the gradient descent process.   
% Algorithm \ref{algo:train_quantized_weight}, dubbed as Learned Quantized Weights (LQW), presents the procedure of our proposed method to train a quantized network weight. 


Specifically, for a general case of representing a network weight $\bW_q$ of $N_w$ elements by $K_w$-bits, we learn a binary weight encoding $\bS_b^w\in\{-1,+1\}^{N_w\times K_w}$ and a quantization basis vector $\bv^w=[v_1^w,\cdots, v_{K_w}^w]\in\bbR^{K_w}$. Consequently, the network weight can be directly replaced by $\bS_b^w\bv^w$ in the cost function, i.e., $\bW_q=\bS_b^w\bv^w$.
% \vspace{-2pt}
\begin{equation}
    \min_{\Theta}\mathcal{L}(\Theta),\quad \textrm{s.t. } \bS_{bi}^w\in\{-1,+1\}^{N_w\times K_w} ~~\forall i,
% \vspace{-2pt}
\end{equation}
where $\Theta=\{\bS_{bi}^w,\bv_i^w\}_{\forall i}$ is the set of all network parameters and $\mathcal{L}$ is a cost function, e.g., cross-entropy for classification. 

\begin{algorithm}[t]
\setlength{\textfloatsep}{-10pt}
\setlength{\floatsep}{-10pt}
\setlength{\intextsep}{0pt}
\caption{\textbf{Learned Quantized Weights (LQW)}.\newline $\mathcal{L}$ is the  cost function for a mini-batch.}\label{algo:train_quantized_weight}
\SetKwInOut{Requires}{Requires}
\SetKwInOut{Output}{Output}
\SetKwInOut{Parameters}{Parameters}
\Requires{Learning rate $\eta$ and learning-rate scaling factors $\{\gamma_{\bv}, \gamma_{\bs}\}$}
\Parameters{Encoding matrix $\bS^w$\hspace{-2pt}, basis vector $\bv^w$}
% \BlankLine
\textbf{Forward propagation:} \\
$\quad\bS_b^w=\sign(\bS^w)$\\
$\quad\bW_q=\bS_b^w\bv^w$\\
\textbf{Backward propagation and Parameter update:}\\
$\quad$Given $\frac{\partial\mathcal{L}}{\partial\bW_q}$ obtained using the chain rule of gradient descent, compute $\frac{\partial\mathcal{L}}{\partial\bS_b^w}$ and $\frac{\partial\mathcal{L}}{\partial\bv^w}$\\
$\quad\bv^w\gets\bv^w - \gamma_\bv\eta\frac{\partial\mathcal{L}}{\partial\bv^w}$\\
$\quad\bS^w\gets\textrm{clip}\left(\bS^w - \gamma_\bs\eta\frac{\partial\mathcal{L}}{\partial\bS_b^w}, -1, 1\right)$ ~~~~~~~~~~\tcp{STE}
\end{algorithm}

To handle the binary constraint on the weight encoding $\bS_b^w$, inspired by \cite{BinaryConnect}, we 
% only binarize $\bS^w$  during the forward (i.e., using $\sign$ function) and backward propagations, and 
introduce a full-precision encoding matrix $\bS^w$ (i.e., $\bS^w\in\bbR^{N_w\times K_w}$) for parameter updates, and obtain $\bS_b^w$ using $\sign$ function (i.e., $\bS_b^w=\sign(\bS^w)$) only during forward and backward propagations.
Furthermore, in order to update $\bS^w$ using gradient descent, we adopt the straight-through estimator (STE) $\frac{\partial\sign(z)}{\partial z}=1_{|z|\le 1}$ \cite{STE}, i.e., $\frac{\partial \mathcal{L}}{\partial \bS_b^w}=\frac{\partial \mathcal{L}}{\partial \bS^w}$ for $\bS^w\in[-1, 1]$, to approximate the gradients propagating through the $\sign$ function. 
Regarding the quantization basis vectors $\bv^w$, as they have no constraint, they can be updated normally using the standard gradient descent process.
The proposed method allows the quantized weights \red{with learnable quantization levels} to be updated (via the weight encodings and the quantization basis vectors) such that they directly minimize the final cost function through the gradient descent process. Additionally, we want to emphasize that other works (e.g., LQ-Nets, TBN) achieve quantized weights from FP weights during a joint training process. More specifically, their FP weights are updated via back-propagation, while the quantized weights ($\bW_q$) are updated to minimize the $\ell_2$-loss with the learning FP weights (i.e., $\arg\min_{\bW_q}\|\bW_q-\bW\|^2$). This process potentially causes training mismatch, as the gradients cannot directly affect the quantized weights.   

Algorithm \ref{algo:train_quantized_weight}, dubbed as Learned Quantized Weights (LQW), presents the procedure of our proposed method to train a quantized network weight. 
Note that, to maximize the flexibility of the low bit-width CNN, while ensuring its compatibility with bitwise operations, we learn one quantization basis vector and weight encoding per filter.


% In our work, by using an encoding $\bS^w$ and a quantization basis vector $\bv^w$, to construct the quantized weight $\bW_q=\bS_b^w\bv^w$ with $\bS_b^w=\sign(\bS^w)$, $\bS^w$ and $\bv^w$ can be updated via back-propagation. Hence, the gradients can directly affect the quantized weights.

\begin{figure*}[ht]
\centering
% \begin{subfigure}[b]{0.24\textwidth}
% \includegraphics[width=\textwidth]{fig/batchnorm_scale.png}
% \caption{Batch Norm scale}
% \label{fig:batchnorm_scale}
% \end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth]{fig/2nd_quant.png}
\caption{$2$-nd quant. level}
\label{fig:2nd_quant}
\end{subfigure}
% $\qquad$
~~
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth]{fig/3rd_quant.png}
\caption{$3$-rd quant. level}
\label{fig:3rd_quant}
\end{subfigure}
% $\qquad$
~~
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth]{fig/4th_quant.png}
\caption{$4$-th quant. level}
\label{fig:4th_quant}
\end{subfigure}
~~
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth]{fig/MSE_relative_change.png}
\caption{MSE relative changes}
\label{fig:mse_change}
\end{subfigure}
\vspace{-3pt}
\caption[Fig. \ref{fig:2nd_quant}, \ref{fig:3rd_quant}, and \ref{fig:4th_quant} are respectively the distributions of the optimal $2$-nd, $3$-rd, and $4$-th channel-wise quantization levels of the first activation layer of AlexNet with $K_a=2$.
{\small\color{red}\ding{116}} indicates the proposed channel-wise averaged quantization levels - Mean Square Error (MSE) = $7.376$ (using 100 random ImageNet images); and {\small\color{blue}\ding{116}} indicates the quantization levels when considering the whole activation as the input for a scalar quantizer (called as baseline)
- MSE = $6.664$.  
Fig. \ref{fig:mse_change} shows the histogram of the relative changes (\%) in channel-wise MSE of our method compared to the baseline.
% Firstly, we can observe that the optimal quantization levels of different channels vary a lot.
We can observe that, in the baseline approach, the quantization levels tend to be biased toward large values. Although our proposed method results in higher quantization error overall (i.e., $7.376>6.664$), the majority of channels (68 out of 96 channels in Fig. \ref{fig:mse_change}) achieve smaller quantization errors (the relative changes $<0$) compared to the baseline.]
{
Fig. \ref{fig:2nd_quant}, \ref{fig:3rd_quant}, and \ref{fig:4th_quant} are respectively the distributions of the optimal $2$-nd, $3$-rd, and $4$-th channel-wise quantization levels of the first activation layer of AlexNet with $K_a=2$.
{\small\color{red}\ding{116}} indicates the proposed channel-wise averaged quantization levels - Mean Square Error (MSE) = $7.376$ (using 100 random ImageNet images); and {\small\color{blue}\ding{116}} indicates the quantization levels when considering the whole activation as the input for a scalar quantizer (e.g., \protect\cite{LQNets}) (called as baseline)
- MSE = $6.664$.  
Fig. \ref{fig:mse_change} shows the histogram of the relative changes (\%) in channel-wise MSE of our method compared to the baseline.
% Firstly, we can observe that the optimal quantization levels of different channels vary a lot.
We can observe that, in the baseline approach, the quantization levels tend to be biased toward large values. Although our proposed method results in higher quantization error overall (i.e., $7.376>6.664$), the majority of channels (68 out of 96 channels in Fig. \ref{fig:mse_change}) achieve smaller quantization errors (the relative changes $<0$) compared to the baseline.
}
\label{fig:CAQ}
\vspace{-8pt}
\end{figure*}

\begin{algorithm}[!t]
% \setlength{\textfloatsep}{0.cm}
% \setlength{\floatsep}{0.cm}
% \setlength{\intextsep}{0pt}
\caption{\textbf{Channel-wise Averaged Quantizer (CAQ)}. $\mathcal{L}$ is a cost function for a mini-batch.}\label{algo:train_act_quantizer} 
\SetKwInOut{Requires}{Requires}
\SetKwInOut{Parameters}{Parameters}
\SetKwInOut{Input}{Inputs}
\SetKwInOut{Output}{Outputs}
\Input{A mini-batch activation $\bA$ with $C$ channels, Moving-average factor $\mu$, and number of iteration $T$.}
\Output{The quantized activation  $\bA_q$.}
\Parameters{A set of quant. basis vectors $\{\bv^{(j)}\}_{j=1}^C$. }
% \BlankLine
\If{ in the training stage, }{
\textbf{Forward propagation:} \\
\For
% (\tcp*[h]{Compute and update Channel-wise quantizers})
{$j=1$ \KwTo $C$} {
    Set $\bv_0^{(j)} = \bv^{(j)}$ \\
    \For{$t=1$ \KwTo $T$}{
    Given $\bv_{t-1}^{(j)}$, compute $\bS_{t}^{(j)}$ by looking up the index of the nearest quant. level;\\
    Given $\bS_{t}^{(j)}$, compute $\bv_{t}^{(j)}$ by using Eq. \ref{eq:update_v}.
    } 
    % Obtain $\bc_m^\ast$ by alternatively update $\bS$ and $\bc$ for $m$-th channel;\\
    $\bv^{(j)}\gets (1-\mu)\bv_{T}^{(j)}+\mu\bv^{(j)}$\\
}
$\bv^a\hspace{-1pt}=\hspace{-1pt}\frac{1}{C}\hspace{-1pt}\sum_{j=1}^C\hspace{-2pt}\bv^{(j)}$\\
%\tcp{\hspace{-3pt}Channel-wise\hspace{-2pt} Average}
Compute $\bA_q$ by looking up the nearest quantization level 
 $\in \bv^a$ for each element.\\
\textbf{Backward propagation:}\\
Given $\frac{\partial\mathcal{L}}{\partial\bA_q}$ obtained using back-propagation;\\
$\frac{\partial \mathcal{L}}{\partial \bA}= \frac{\partial \mathcal{L}}{\partial \bA_q}\quad$ ~~~~~~~~~~~~~~~~~~~\tcp{STE}
}
\Else(\tcp*[h]{inference stage}){
$\bv^a=\frac{1}{C}\sum_{j=1}^C\bv^{(j)}$ %~~~~~~\tcp{Can be pre-computed}
\\
Compute $\bA_q$ by looking up the nearest quantization level $\in \bv^a$ for each element.\\
}
\end{algorithm}

% \vspace{-2pt}
\subsection{Activation Channel-Wise Averaged Quantizer}
\label{sec:act_quant}
%
% \begin{wrapfigure}{r}{0.46\textwidth}
% \begin{figure}
% \vspace{-1.5em}
% \centering
% \includegraphics[width=0.4\textwidth]{fig/asymmetric_distribution.png}
% \caption{Comparison between 2-bit scalar quantizers using $k$-means, our proposed $(k-1)$-means, and LQ-Nets method. Markers indicate the quantization levels of different methods. The marker of the first quantization level of LQ-Nets is overlapped by a marker of $(k-1)$-means, as both are 0.
% }
% \label{fig:compare_quantizer}
% \vspace{-0.7em}
% % \end{wrapfigure}
% \end{figure}


% \textbf{Scalar quantization using $(k-1)$-means.} 
% \vspace{-2pt}
% \textbf{}
\paragraph{Scalar Quantizer.}
Given a full-precision ReLU activation $\bA\hspace{-0.5pt}\in\hspace{-0.5pt}\bbR_{\ge 0}^{B\times C\times W\times H}$ (i.e., the set of non-negative real values), our goal is to represent $\bA$ using $K_a$-bits with minimized information loss. %A simple method is to perform  scalar quantization to the activations.
We consider $\bA$ as a vector $\ba$ of $N_a$-dimension ($N_a\hspace{-1pt}=\hspace{-1pt}BCWH$). %Similar to \cite{LQNets}, 
We aim to find an optimal quantization basis vector $\bv^a\hspace{-1pt}=\hspace{-1pt}[v_1^a,\cdots,v_{K_a}^a]\hspace{-1pt}\in\hspace{-1pt}\bbR^{K_a}$ and an optimal binary encoding $\bS^a\in\{0,1\}^{N_a\times K_a}$ that minimize the following quantization error:
% \vspace{-2pt}
\begin{equation}
\label{eq:act_quantizer}
    \arg\min_{\bv^a,\bS^a}\|\ba-\bS^a\bv^a\|_2^2,\quad\textrm{s.t. }\bS^a\in\{0,1\}^{N_a\times K_a}.
% \vspace{-2pt}
\end{equation}
This problem can be solved by alternatively updating $\bS^a$ and $\bv^a$:
%
\textbf{\textit{(i)}} Given $\bv^a$ fixed, the optimal $\bS^a$ can be found by looking up the index of the nearest quantization level. 
Note that, for a $K_a$-bit quantization, there are $2^{K_a}$ quantization levels $\bq^a=[q_i^a,\cdots,q_{2^{(K_a)}}^a]\in\bbR^{2^{(K_a)}}$ and 
% \begin{equation}
    $q_i^a = \left\langle\text{Dec2Bin}_{K_a}(i), \bv^a\right\rangle,$
% \end{equation} 
where $\langle\cdot\rangle$ is a dot product and $\text{Dec2Bin}_{K_a}(i)$ is the function convert the decimal value $i$ ($0\le i<2^{K_a})$ to the equivalent $K_a$-bit binary vector, e.g., $\text{Dec2Bin}_{3}(6)=[0, 1, 1]$.
% (most significant bit is the $K_a$-th element of the vector). 
% Additionally, without loss of generality, we assume that $v_1^a<v_2^a<\cdots<v_{K_a}^a$.
%
\textbf{\textit{(ii)}} Given $\bS^a$ fixed, we have the closed-form solution for $\bv^a$ as follows: 
% \vspace{-2pt}
\begin{equation}
\label{eq:update_v}
\bv^a = ({\bS^a}^\top\bS^a)^{-1}{\bS^a}^\top\ba.   
% \vspace{-2pt}
\end{equation}
% Once the quantization level vector is learned, the quantized activation can be obtained by looking up the nearest quantization level for each value of $\bA$.

% For convenience, we name the scalar quantization method of Eq. \ref{eq:act_quantizer} as ``$(k-1)$-means'' to emphasize the fact that, slightly different from standard $k$-means, we only need to learn $(k-1)$ centroids (one centroid is fixed, i.e., $c_1=0$).
% Once the quantization level vector is learned, the quantized activation can be obtained by looking up the nearest quantization level for each value of $\ba$:
% \begin{equation}
% \label{eq:lookup}
% a_q=c_j, ~\textrm{where}~c_j=\min_j\|a-c_j\|_2^2.
% % \vspace{-0.5em}
% \end{equation}

% % Importantly, we note that a $2^K$-bit vector $\bs_i$ can be equivalently represented by $K$-bit vector during inference time, e.g., for $K=2$, $[1,0,0,0]\to [-1,-1];[0,1,0,0]\to [-1,+1];[0,0,1,0]\to [+1,-1];[0,0,0,1]\to [+1,+1]$. We now show how the dot product a quantized weight and activation can be computed by bitwise operations.
% % \begin{equation}
% %     \sum_{i=1}^{K_w}\sum_{j=1}^{K_a}\bB_{i,j}()
% % \end{equation}


% We note that the proposed quantizer in LQ-Nets \cite{LQNets} shares certain similarity to our approach, i.e., trying to minimize the quantization error. Differently, for $K$-bit quantization, LQ-Nets learns a basis vector $\bv=[v_1,\cdots,v_K]$ of $K$ scalars. Then, the $2^K$ quantization levels are computed from $\bv$ (e.g., $\{0, v_1, v_2, v_1+v_2\}$ for $K=2$). However, we found that LQ-Nets  method is sub-optimal for asymmetric inputs, e.g., ReLU activation.
% Figure \ref{fig:compare_quantizer} presents comparison between scalar quantizers using our proposed $(k-1)$-means and using the LQ-Nets proposed method \cite{LQNets} with the output of 1-st ReLU activation layer of AlexNet using 10 random ImageNet images. 
% We can clearly observe that LQ-Nets quantizer is sub-optimal and results in much larger quantization error (Mean Square Error (MSE)) in comparison to our $(k-1)$-means quantizer. 
% Additionally, our $(k-1)$-means quantizer only has a slightly-higher quantization error than the optimal $k$-means does.
% The comparison can clearly demonstrate the advantage of our proposed method.

%man: what are these weight and activation? e.g. which network / layer?
%man: are kmeans and LQ-nets using same bit-width in this example?
% \begin{figure}[t]
% \centering
% \begin{subfigure}[b]{0.30\textwidth}
% \includegraphics[width=\textwidth]{fig/symmetric_distribution.png}
% \caption{Weight}
% \label{fig:weight_dist}
% \end{subfigure}
% $\qquad$
% \begin{subfigure}[b]{0.30\textwidth}
% \includegraphics[width=\textwidth]{fig/asymmetric_distribution.png}
% \caption{ReLU activation}
% \label{fig:act_dist}
% \end{subfigure}
% \caption{Comparison between 2-bit scalar quantizers using our proposal and using the LQ-Nets proposal \cite{LQNets}. For symmetric distribution, e.g., the weight of 2-nd conv. layer of AlexNet in Fig. \ref{fig:weight_dist}, LQ-Nets quantizer achieves similar Mean Square Quantization Errors (MSE) with $k$-means. However, for the asymmetric distribution, e.g., the output of 1-st ReLU activation layer of AlexNet with 10 random ImageNet images in Fig. \ref{fig:act_dist}, LQ-Nets quantizer is sub-optimal and results in much larger quantization error in comparison to our $(k-1)$-means quantizer. 
% % We also observe a small increase of quantization error of our proposal in comparison with $k$-means.
% }
% \label{fig:compare_quantizer}
% \end{figure}
%
% \noindent\textbf{Channel-wise averaged quantization.} 
\paragraph{Channel-Wise Averaged Quantization.}
The Batch Normalization layer \cite{batch_norm} includes two steps: {{(i)}} normalizing and {{(ii)}} shifting and scaling. While the normalizing step tries to make each channel of $\bA$ to have zero-mean and unit-variance, the scaling and shifting step makes the variances of channels different. The variances can be very large or very small, depending on the corresponding scaling factor of the $i$-th channel.
Hence, when a single scalar quantizer is used for $\bA$ as in previous works (e.g., LQ-Nets \cite{LQNets}) (called as baseline), few channels which have high variances can significantly affect the quantization basis values. Consequently, the resulting quantization basis vector potentially causes significant information loss in many channels with low variances, which cumulatively have noticeable impacts on outputs. 
Additionally, slightly less focus on large activation values might help to reduce overfitting.
%
%
To address this problem, first, we propose to learn a scalar quantizer for each channel of activation $\bA$. Then, the quantization basis values for the layer-wise quantizer can be obtained by taking the average of all quantization basis values of channel-wise quantizers, i.e., $v_i^a=\frac{1}{C}\sum_{j=1}^Cv_i^{a(j)},$  where $v_i^{a(j)}$ is the $i$-th quantization basis value of $j$-th channel. With this proposed approach, the layer-wise quantization levels minimize the quantization errors on the majority of channels. 
Figure \ref{fig:CAQ} provides an example to illustrate our proposed method.
%
Besides, noticeably, only a mini-batch of input is available at each forward/backward step, we necessarily apply exponential moving average to update the channel-wise quantization level vectors to ensure stability.
Algorithm \ref{algo:train_act_quantizer}, dubbed as Channel-wise Averaged Quantizer (CAQ), summarizes the procedure for training and inference of our proposed quantizer for activations. Note that during inference, only the channel-wise averaged quantizer is required. Hence, our method has the same time complexity as the baseline does.


==> [IJCAI20_camera_ready] Network quantization/tex/related_works.tex <==
% \vspace{-3pt}
\section{Related Works}
How to improve inference efficiency of CNN for practical applications has been an active research field. % and attracts abundant research efforts.
Existing approaches can be roughly divided into three main categories: {compact network design},
% \cite{net_in_net,SqueezeNet,MobileNets,ShuffleNet,GoogLeNet,MorphNet}, 
{parameter reduction,} 
% (including low-rank approximation  \cite{predict_param,linear_structure,low_rank_expansion,CP-Decomposition,tensorizing,8099498,accelerateCNN,LessIsMore} 
% and {connection pruning}), %\cite{DeepCompression,LBWC,channel_pruning,ThiNet,NetworkSlimming,nips,Learning-Compression,FasterGP,discrimiation_aware_prunning}), 
and {network quantization}. In this section, we discuss recent works on the last category, to which our work belongs.

% \textbf{Weight-only quantization.} 
\paragraph{Weight-only Quantization.}
Earlier works have applied the basic form of weight quantization to directly constrains the weight values into the binary space without or with a scaling factor, i.e., $\{-1, 1\}$ in BinaryConnect \cite{BinaryConnect} or $\{-\alpha, \alpha\}$ in Binary-Weight-Networks (BWN) \cite{xnor_net}. 
Ternary Weight Networks (TWN) \cite{TWN} proposed to quantize weights into a ternary form of $\{-\alpha, 0, \alpha\}$. Trained Ternary Quantization (TTQ) \cite{TTQ} generalized TWN by constraining the weights to asymmetric ternary values $\{-\alpha_n, 0, \alpha_p\}$. In comparison to the binary weights, the ternary weights can help to improve performance, while achieving a similar speedup during inference \cite{tbn}. 
% \cite{netcompress_vec_quant} applied scalar quantization using $k$-means to quantize pre-trained network weights.
\citeauthor{lossaware} proposed loss-aware quantized networks which can further improve the accuracy by considering the loss in learning the binary/ternary weights. \citeauthor{INQ} presented incremental network quantization (INQ) to incrementally convert a pre-trained FP CNN model to a low-precision one.
% whose weights are constrained to be either power of two or zero. 
% \cite{TNN_truncatedGauusianApprox} proposed a gradient correctness optimization method in straight-through-estimator design, which can help to reduce accuracy drops of ternary weight networks.

% \vspace{-2pt}
% \textbf{Weight and Activation quantization.}
\paragraph{Weight and Activation Quantization.}
Since quantization of activations can substantially reduce complexity further, by allowing the dot products to be implemented with bit-wise operations (i.e., ${xor}$ and ${popcount}$) \cite{BinaryNet,xnor_net}, this approach attracts more and more attention \cite{xnor_net,dorefa,LQNets}. 
In early works \cite{BinaryNet,xnor_net}, the authors proposed to binarize both weights and activations to $\{-1,1\}$. Although these methods can be highly efficient in reference time, there are considerable accuracy drops compared to FP networks. 
% \vspace{-2pt}
To address this problem, the generalized low bit-width quantization was further studied in \cite{dorefa,log_data_represent}. By allowing to use more bits, this approach can provide a trade-off between accuracy and inference complexity.
A popular choice of  early works is the uniform quantization \cite{dorefa,QNN}.
\citeauthor{log_data_represent} later proposed logarithmic quantization which can help to improve the inference efficiency via bit-shift operations. 
\citeauthor{weighted_entropy} used weighted-entropy to learn quantizers that are more concentrated on the values that are neither too small nor too large.
\citeauthor{hwgq} proposed to pre-compute a single activation quantizer for all activation layers by fitting the probability density function of a half-wave Gaussian distribution. 
% \citeauthor{HORQ} proposed High-Order Residual Quantization framework, which binarizes FP values and residuals to achieve more accurate approximation. \citeauthor{dsq} proposed  Differentiable Soft Quantization (DSQ) which uses smooth differentiable quantization function, instead of the discrete quantization, at the beginning and evolve during training to gradually approximate the standard discrete quantization. 
As opposed to the fixed, handcrafted quantization schemes of the aforementioned works, LQ-Nets \cite{LQNets} proposed to jointly train a quantized CNN and its associated quantizers.
\citeauthor{QIL} proposed to train quantizers with parameterized intervals, which simultaneously performs both pruning and clipping. \citeauthor{bonn} proposed  Bayesian optimized
1-bit CNNs (BONN) which incorporates the prior distributions of FP kernels and features into the Bayesian framework to construct 1-bit CNNs.
%
% Besides, recently, many works have been also proposed to tackle the difficulty of training DNN with low-bitwidth weights and activations, such as two step quantization \cite{TwoStepQF}, two-stage optimization, progressive quantization, and guided training \cite{guidedQuantize}. 
% \vspace{-2pt}
Besides, recent works on designing new structures for binary networks achieve  promising results.
Bi-Real Net \cite{bi-real} introduced a new variant of residual structure to preserve the real activations before the $\sign$ function. The shortcut can help to increase the representational capability of the 1-bit convolutional block. 
% \red{BBG \cite{BBG} further improves the residual connection in Bi-Real Net with a gated residual, which additionally learns the channel attention.}
%($\sign$ $\to$ 1-bit convolution $\to$ batch norm $\to$ addition operator). 
% ABC-Net \cite{NIPS2017_6638} adopts multiple binary weights and activations to approximate full-precision weights such that the prediction accuracy degradation can be alleviated. 
\citeauthor{groupnet} proposed Group-Net, in which a set of binary convolution branches can effectively replace a FP convolution.
%a full-precision convolutional group can be effectively 
% reconstructed by aggregating a set of binary branches. 
% replaced by a set of binary branches.
% Binary Ensemble Neural Network \cite{binary_ensemble_NN} aggregated multiple binary networks by boosting or bagging.

% \textbf{Weight, Activation, and Gradient quantization.}
% Quantizing gradients, in addition to quantizing weights and activations, have been explored in DoReFa-Net \cite{dorefa}, TernGrad \cite{TernGrad}, WAGE \cite{wage}. Those methods are very beneficial not only for inference, but also for faster training including reduction in gradient transferring overhead in distributed training. However, quantizing gradients has a significant impact on learning process and generally results in large performance drops. Hence, this is not the main focus of this work.



==> ijcai20bib <==


@InProceedings{zhou:2018,
author = {Yiren Zhou and Seyed-Mohsen Moosavi-Dezfooli and  Ngai-Man Cheung and Pascal Frossard},
title = {Adaptive Quantization for Deep Neural Network},
booktitle = {AAAI},
year = {2018},
pages={4596--4604},
}


@InProceedings{Yang_2019_CVPR,
author = {Yang, Jiwei and Shen, Xu and Xing, Jun and Tian, Xinmei and Li, Houqiang and Deng, Bing and Huang, Jianqiang and Hua, Xian-sheng},
title = {Quantization Networks},
booktitle = {CVPR},
year = {2019},
pages={7300-7308},
}

@INPROCEEDINGS{RBCN,
  title={{Rectified Binary Convolutional Networks for Enhancing the Performance of 1-bit DCNNs}},
  author={Chunlei Liu and Wenrui Ding and Xin Xia and Yuan Hu and Baochang Zhang and Jianzhuang Liu and Bohan Zhuang and Guodong Guo},
  booktitle={IJCAI},
  year={2019},
  pages= {854--860},
}

@INPROCEEDINGS{BBG, 
author={M. {Shen} and X. {Liu} and R. {Gong} and K. {Han}},
booktitle={ICASSP}, 
title={Balanced Binary Neural Networks with Gated Residual}, 
year={2020}}

@INPROCEEDINGS{MobileNetV2, 
author={Mark Sandler and Andrew Howard and Menglong Zhu and Andrey Zhmoginov and Liang-Chieh Chen},
booktitle={CVPR}, 
title={{MobileNetV2: Inverted Residuals and Linear Bottlenecks}}, year={2018}, 
pages={4510-4520},
}



@inproceedings{TernGrad,
 author = {Wen, Wei and Xu, Cong and Yan, Feng and Wu, Chunpeng and Wang, Yandan and Chen, Yiran and Li, Hai},
 title = {TernGrad: Ternary Gradients to Reduce Communication in Distributed Deep Learning},
 booktitle = {NIPS},
 year = {2017},
} 

@inproceedings{pcnn,
  title={Projection Convolutional Neural Networks for 1-bit CNNs via Discrete Back Propagation},
  author={Jiaxin, Gu and Ce, Li and Baochang, Zhang and Jungong, Han and Xianbin, Cao and Jianzhuang, Liu and David, Doermann},
  booktitle={AAAI},
  year={2019}
}

@inproceedings{bonn,
  title={{Bayesian Optimized 1-bit CNNs}},
  author={Gu, Jiaxin and Zhao, Junhe and Jiang, Xiaolong and Zhang, Baochang and Liu Jianzhuang and Guo, Guodong and Ji, Rongrong},
  booktitle={ICCV},
  year={2019},
  pages={4909-4917}
}

@InProceedings{dsq,
    title={Differentiable Soft Quantization: Bridging Full-Precision and Low-Bit Neural Networks},
    author={Gong, Ruihao and Xianglong Liu and Shenghu Jiang and Tianxiang Li and Peng Hu and Jiazhen Lin and Fengwei Yu and Junjie Yan},
    year={2019},
    pages = {4852-4861},
    booktitle={ICCV},
}

@article{wage,
  author    = {Shuang Wu and
               Guoqi Li and
               Feng Chen and
               Luping Shi},
  title     = {Training and Inference with Integers in Deep Neural Networks},
  booktitle = {ICLR},
  year      = {2018},
}


@InProceedings{MorphNet,
author = {Gordon, Ariel and Eban, Elad and Nachum, Ofir and Chen, Bo and Wu, Hao and Yang, Tien-Ju and Choi, Edward},
title = {MorphNet: Fast \& Simple Resource-Constrained Structure Learning of Deep Networks},
booktitle = {CVPR},
year = {2018}
}

@inproceedings{netcompress_vec_quant,
  author    = {Yunchao Gong and
               Liu Liu and
               Ming Yang and
               Lubomir D. Bourdev},
  title     = {Compressing Deep Convolutional Networks using Vector Quantization},
  booktitle={ICLR Workshop},
  year={2015}
}

@inproceedings{TNN_truncatedGauusianApprox,
  author    = {Zhezhi He and
               Deliang Fan},
  title     = {{Simultaneously Optimizing Weight and Quantizer of Ternary Neural Network
               using Truncated Gaussian Approximation}},
  booktitle={CVPR},
  year={2019}
}


@inproceedings{groupnet,
  author    = {Bohan Zhuang and
               Chunhua Shen and
               Mingkui Tan and
               Lingqiao Liu and
               Ian D. Reid},
  title     = {{Structured Binary Neural Networks for Accurate Image Classification and Semantic Segmentation}},
    booktitle={CVPR},
  year={2019},
  pages={413--422},
}

@inproceedings{binary_ensemble_NN,
  author    = {Shilin Zhu and
               Xin Dong and
               Hao Su},
  title     = {{Binary Ensemble Neural Network: More Bits per Network or More Networks per Bit?}},
  booktitle={CVPR},
  year={2019}
}


@inproceedings{CBCN,
  title={{Circulant Binary Convolutional Networks: Enhancing the Performance of 1-bit DCNNs with Circulant Back Propagation}},
  author={Liu, Chunlei and Ding, Wenrui and Gu, Jiaxin and Zhang, Baochang and Ji, Rongrong and Liu, Jianzhuang},
  booktitle={CVPR},
  year={2019}
}

@InProceedings{QIL,
author = {Jung, Sangil and Son, Changyong and Lee, Seohyung and Son, Jinwoo and Han, Jae-Joon and Kwak, Youngjun and Hwang, Sung Ju and Choi, Changkyu},
title = {Learning to Quantize Deep Networks by Optimizing Quantization Intervals With Task Loss},
booktitle = {CVPR},
year = {2019},
pages = {4350--4359},
}

@InProceedings{OQI,
  author    = {Sangil Jung and
               Changyong Son and
               Seohyung Lee and
               JinWoo Son and
               Youngjun Kwak and
               Jae{-}Joon Han and
               Changkyu Choi},
  title     = {{Joint Training of Low-Precision Neural Network with Quantization Interval Parameters}},
booktitle = {CVPR},
  year      = {2019},
}

@InProceedings{bi-real,
author = {Liu, Zechun and Wu, Baoyuan and Luo, Wenhan and Yang, Xin and Liu, Wei and Cheng, Kwang-Ting},
title = {{Bi-Real Net: Enhancing the Performance of 1-bit CNNs with Improved Representational Capability and Advanced Training Algorithm}},
booktitle = {ECCV},
year = {2018},
pages={747--763},
}

@incollection{discrimiation_aware_prunning,
title = {{Discrimination-aware Channel Pruning for Deep Neural Networks}},
author = {Zhuang, Zhuangwei and Tan, Mingkui and Zhuang, Bohan and Liu, Jing and Guo, Yong and Wu, Qingyao and Huang, Junzhou and Zhu, Jinhui},
booktitle = {NIPS},
pages = {875--886},
year = {2018},
}


@incollection{NIPS2017_6638,
title = {{Towards Accurate Binary Convolutional Neural Network}},
author = {Lin, Xiaofan and Zhao, Cong and Pan, Wei},
booktitle = {NIPS},
pages = {345--353},
year = {2017},
}


@InProceedings{LessIsMore,
author="Zhou, Hao
and Alvarez, Jose M.
and Porikli, Fatih",
editor="Leibe, Bastian
and Matas, Jiri
and Sebe, Nicu
and Welling, Max",
title={{Less Is More: Towards Compact CNNs}},
booktitle="ECCV",
year="2016",
}

@article{log_data_represent,
  author    = {Daisuke Miyashita and
               Edward H. Lee and
               Boris Murmann},
  title     = {{Convolutional Neural Networks using Logarithmic Data Representation}},
  journal   = {CoRR},
  volume    = {abs/1603.01025},
  year      = {2016},
}

@InProceedings{explicit_lossaware,
author = {Zhou, Aojun and Yao, Anbang and Wang, Kuan and Chen, Yurong},
title = {{Explicit Loss-Error-Aware Quantization for Low-Bit Deep Neural Networks}},
booktitle = {CVPR},
month = {June},
year = {2018}
}

@article{dropout,
 author = {Srivastava, Nitish and Hinton, Geoffrey and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
 title = {{Dropout: A Simple Way to Prevent Neural Networks from Overfitting}},
 journal = {JMLR},
 issue_date = {January 2014},
 volume = {15},
 number = {1},
 month = jan,
 year = {2014},
 pages = {1929--1958},
} 


@InProceedings{xavier_init,
  title = 	 {Understanding the difficulty of training deep feed-forward neural networks},
  author = 	 {Xavier, Glorot and Yoshua, Bengio},
  booktitle = 	 {AISTATS},
  year = 	 {2010},
}

@article{QNN,
 author = {Hubara, Itay and Courbariaux, Matthieu and Soudry, Daniel and El-Yaniv, Ran and Bengio, Yoshua},
 title = {{Quantized Neural Networks: Training Neural Networks with Low Precision Weights and Activations}},
 journal = {JMLR},
 year = {2017},
 pages = {6869–6898},
 volume = {18},
number = {1},
} 

@inproceedings{INQ,
title={{Incremental Network Quantization: Towards Lossless CNNs with Low-Precision Weights}},
author={Aojun, Zhou and Anbang, Yao and Yiwen, Guo and Lin, Xu and Yurong, Chen},
booktitle={ICLR},
year={2017},
}

@InProceedings{DL_limited_num_precision,
  title = 	 {{Deep Learning with Limited Numerical Precision}},
  author = 	 {Suyog Gupta and Ankur Agrawal and Kailash Gopalakrishnan and Pritish Narayanan},
  booktitle = 	 {ICML},
  year = 	 {2015},
  pages = {1737–1746},
}

@inproceedings{NN_few_mul,
  title={{Neural Networks with Few Multiplications}},
  author={Zhouhan Lin and Matthieu Courbariaux and Roland Memisevic and Yoshua Bengio},
 booktitle = {ICML},
 year = {2016},
}

@inproceedings{fix_point_quant,
 author = {Darryl D. Lin and Sachin S. Talathi and V. Sreekanth Annapureddy},
 title = {{Fixed Point Quantization of Deep Convolutional Networks}},
 booktitle = {ICML},
 year = {2016},
 pages = {2849–2858},
} 

@incollection{BinaryConnect,
title = {{BinaryConnect: Training Deep Neural Networks with binary weights during propagations}},
author = {Courbariaux, Matthieu and Bengio, Yoshua and David, Jean-Pierre},
booktitle = {NIPS},
pages = {3123--3131},
year = {2015},
}

@inproceedings{8bit_parallel,
  author    = {Tim Dettmers},
  title     = {8-BIT APPROXIMATIONS FOR PARALLELISM IN DEEP LEARNING},
  booktitle={ICLR},
  year      = {2016},
}

@inproceedings{TWN,
  author    = {Fengfu Li and
               Bin Liu},
  title     = {Ternary Weight Networks},
  booktitle={ICLR},
  year      = {2017},
}

@inproceedings{batch_norm,
 author = {Ioffe, Sergey and Szegedy, Christian},
 title = {Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift},
 booktitle = {ICML},
 year = {2015},
 pages = {448–456},
} 

@InProceedings{lossaware17,
	title={Loss-aware Binarization of Deep Networks},
	author={Hou, Lu and Yao, Quanming and Kwok, James T.},
	booktitle={ICLR},
	year={2017}
}

@inproceedings{lossaware,
title={Loss-aware Weight Quantization of Deep Networks},
author={Lu Hou and James T. Kwok},
booktitle={ICLR},
year={2018},
}

@inproceedings{FasterGP,
  title={{Faster gaze prediction with dense networks and Fisher pruning}},
  author={Lucas Theis and Iryna Korshunova and Alykhan Tejani and Ferenc Husz{\'a}r},
 booktitle = {ECCV},
month = {June},
year = {2018}
}

@InProceedings{Learning-Compression,
author = {Carreira-Perpinan, Miguel A. and Idelbayev, Yerlan},
title = {{“Learning-Compression” Algorithms for Neural Net Pruning}},
booktitle = {CVPR},
year = {2018}
}

@inproceedings{NetworkSlimming,
	title = {Learning Efficient Convolutional Networks through Network Slimming},
	author = {Liu, Zhuang and Li, Jianguo and Shen, Zhiqiang and Huang, Gao and Yan, Shoumeng and Zhang, Changshui},
	booktitle = {ICCV},
	year = {2017}
}

@InProceedings{nips,
author = {Yu, Ruichi and Li, Ang and Chen, Chun-Fu and Lai, Jui-Hsin and I. Morariu, Vlad and Han, Xintong and Gao, Mingfei and Lin, Ching-Yung and Davis, Larry},
year = {2018},
booktitle = {CVPR},
title = {{NISP: Pruning Networks using Neuron Importance Score Propagation}}
}

@InProceedings{ThiNet,
  author={Jian-Hao Luo, Jianxin Wu, and Weiyao Lin},
  title={{ThiNet: A Filter Level Pruning Method for Deep Neural Network Compression}},
  booktitle={ICCV},
  year = {2017},
}

@InProceedings{channel_pruning,
author = {He, Yihui and Zhang, Xiangyu and Sun, Jian},
title = {{Channel Pruning for Accelerating Very Deep Neural Networks}},
booktitle = {ICCV},
year = {2017}
}


@inproceedings{LBWC,
 author = {Han, Song and Pool, Jeff and Tran, John and Dally, William J.},
 title = {{Learning Both Weights and Connections for Efficient Neural Networks}},
 booktitle = {NIPS},
 year = {2015},
} 

@article{accelerateCNN,
 author = {Zhang, Xiangyu and Zou, Jianhua and He, Kaiming and Sun, Jian},
 title = {Accelerating Very Deep Convolutional Networks for Classification and Detection},
 journal = {IEEE TPAMI},
 issue_date = {October 2016},
 volume = {38},
 number = {10},
 year = {2016},
 pages = {1943--1955},
} 


@inproceedings{tensorizing,
 author = {Novikov, Alexander and Podoprikhin, Dmitry and Osokin, Anton and Vetrov, Dmitry},
 title = {Tensorizing Neural Networks},
 booktitle = {NIPS},
 year = {2015},
} 

@inproceedings{CP-Decomposition,
author = {Lebedev, Vadim and Ganin, Yaroslav and Rakhuba, Maksim and Oseledets, Ivan and Lempitsky, Victor},
year = {2015},
booktitle = {ICLR},
title = {{Speeding-up Convolutional Neural Networks Using Fine-tuned CP-Decomposition}},
}

@inproceedings{low_rank_expansion,
  title={Speeding up Convolutional Neural Networks with Low Rank Expansions},
  author={Max Jaderberg and Andrea Vedaldi and Andrew Zisserman},
  booktitle={BMVC},
  year={2014},
}

@inproceedings{linear_structure,
 author = {Denton, Emily and Zaremba, Wojciech and Bruna, Joan and LeCun, Yann and Fergus, Rob},
 title = {{Exploiting Linear Structure Within Convolutional Networks for Efficient Evaluation}},
 booktitle = {NIPS},
 year = {2014},
} 


@inproceedings{predict_param,
 author = {Denil, Misha and Shakibi, Babak and Dinh, Laurent and Ranzato, Marc'Aurelio and de Freitas, Nando},
 title = {{Predicting Parameters in Deep Learning}},
 booktitle = {NIPS},
 year = {2013},
} 

@article{GoogLeNet,
  title={Going deeper with convolutions},
  author={Christian Szegedy and Wei Liu and Yangqing Jia and Pierre Sermanet and Scott E. Reed and Dragomir Anguelov and Dumitru Erhan and Vincent Vanhoucke and Andrew Rabinovich},
  journal={CVPR},
  year={2015},
}

@inproceedings{MobileNets,
author = {G. Howard, Andrew and Zhu, Menglong and Chen, Bo and Kalenichenko, Dmitry and Wang, Weijun and Weyand, Tobias and Andreetto, Marco and Adam, Hartwig},
year = {2017},
title = {{MobileNets: Efficient Convolutional Neural Networks for Mobile Vision Applications}},
booktitle = {CVPR},
}

@inproceedings{ShuffleNet,
author = {Zhang, Xiangyu and Zhou, Xinyu and Lin, Mengxiao and Sun, Jian},
year = {2017},
title = {{ShuffleNet: An Extremely Efficient Convolutional Neural Network for Mobile Devices}},
booktitle = {CVPR},
}

@article{SqueezeNet,
  author    = {Forrest N. Iandola and
               Matthew W. Moskewicz and
               Khalid Ashraf and
               Song Han and
               William J. Dally and
               Kurt Keutzer},
  title     = {{SqueezeNet: AlexNet-level accuracy with 50x fewer parameters and {\textless}1MB model size}},
  journal   = {CoRR},
  volume    = {abs/1602.07360},
  year      = {2016},
}


@inproceedings{net_in_net,
  author    = {Min Lin and
               Qiang Chen and
               Shuicheng Yan},
  title     = {Network In Network},
    booktitle = {ICLR},
  year={2014}
}

@inproceedings{TTQ,
  title={{Trained Ternary Quantization}},
  author={Zhu, Chenzhuo and Han, Song and Mao, Huizi and Dally, William J},
  booktitle = {ICLR},
  year={2017}
}

@inproceedings{LQNets,
    author = {Zhang, Dongqing and Yang, Jiaolong and Ye, Dongqiangzi and Hua, Gang},
    title = {{LQ-Nets: Learned Quantization for Highly Accurate and Compact Deep Neural Networks}},
    booktitle = {ECCV},
    year = {2018},
    pages={373--390},
}

@article{TwoStepQF,
  title={{Two-Step Quantization for Low-bit Neural Networks}},
  author={Peisong Wang and Qinghao Hu and Yifan Zhang and Chunjie Zhang and Yang Liu and Jian Cheng},
  journal={CVPR},
  year={2018},
}

@inproceedings{hwgq,
  author = {Zhaowei Cai and Xiaodong He and Jian Sun and Nuno Vasconcelos},
  Title = {{Deep Learning with Low Precision by Half-wave Gaussian Quantization}},
  booktitle = {CVPR},
  pages={5918-5926},
  Year  = {2017}
}

@inproceedings{HORQ,
author = {Li, Zefan and Ni, Bingbing and Zhang, Wenjun and Yang, Xiaokang and Gao, Wen},
year = {2017},
title = {{Performance Guaranteed Network Acceleration via High-Order Residual Quantization}},
booktitle = {ICCV},
pages={2584-2592},
}

@InProceedings{BinaryNet,
author = {Wei Tang and Gang Hua and Liang Wang},
title = {{How to Train a Compact Binary Neural Network with High Accuracy?}},
booktitle = {AAAI},
year = {2017},
pages={2625--2631},
}

@InProceedings{tbn,
author = {Wan, Diwen and Shen, Fumin and Liu, Li and Zhu, Fan and Qin, Jie and Shao, Ling and Tao Shen, Heng},
title = {{TBN: Convolutional Neural Network with Ternary Inputs and Binary Weights}},
booktitle = {ECCV},
year = {2018},
pages={322--339},
}

@InProceedings{BNN,
  title={{BinaryNet: Training Deep Neural Networks with Weights and Activations Constrained to +1 or -1}},
  author={Matthieu Courbariaux and Yoshua Bengio},
  booktitle={NIPS},
  year={2016},
}

@inproceedings{tnn,
author = {Alemdar, Hande and Leroy, Vincent and Prost-Boucle, Adrien and Pétrot, Frédéric},
year = {2017},
title = {{Ternary neural networks for resource-efficient AI applications}},
booktitle = {IJCNN}
}

@InProceedings{xnor_net,
author="Rastegari, Mohammad and Ordonez, Vicente and Redmon, Joseph and Farhadi, Ali",
title={{XNOR-Net: ImageNet Classification Using Binary Convolutional Neural Networks}},
booktitle="ECCV",
year="2016",
pages="525--542",
}

@INPROCEEDINGS{entropy_penalize, 
author={Gabriel Pereyra and George Tucker and Jan Chorowski and Łukasz Kaiser and Geoffrey Hinton}, 
booktitle={ICLR Workshop}, 
title={Regularizing neural networks by penalizing confident output distributions}, 
year={2017}, }


@INPROCEEDINGS{weighted_entropy, 
author={Eunhyeok Park and Junwhan Ahn and Sungjoo Yoo}, 
booktitle={CVPR}, 
title={Weighted-Entropy-Based Quantization for Deep Neural Networks}, 
year={2017}, 
pages={5456--5464},
}

@inproceedings{DeepCompression,
author = {Han, Song and Mao, Huizi and Dally, William},
year = {2016},
booktitle={ICLR},
title = {{Deep Compression: Compressing Deep Neural Networks with Pruning, Trained Quantization and Huffman Coding}}
}

@inproceedings{LearningWeightConnect,
  title={Learning both Weights and Connections for Efficient Neural Networks},
  author={Song Han and Jeff Pool and John Tran and William J. Dally},
  booktitle={NIPS},
  year={2015}
}

@incollection{soft2hard,
title = {Soft-to-Hard Vector Quantization for End-to-End Learning Compressible Representations},
author = {Agustsson, Eirikur and Mentzer, Fabian and Tschannen, Michael and Cavigelli, Lukas and Timofte, Radu and Benini, Luca and Gool, Luc V},
booktitle = {NIPS},
year = {2017},
}

@inproceedings{BinarizedNN,
  title={Binarized Neural Networks},
  author={Itay Hubara and Matthieu Courbariaux and Daniel Soudry and Ran El-Yaniv and Yoshua Bengio},
  booktitle={NIPS},
  year={2016}
}

@article{STE,
author = {Hinton, Geoffreye},
year = {2012},
title = {Neural networks for machine learning},
journal = {Coursera, video lectures}
}

@article{STE1,
  title={Estimating or Propagating Gradients Through Stochastic Neurons for Conditional Computation},
  author={Yoshua Bengio and Nicholas L{\'e}onard and Aaron C. Courville},
  journal={CoRR},
  year={2013},
  volume={abs/1308.3432}
}

@book{info_theory,
 author = {Cover, Thomas M. and Thomas, Joy A.},
 title = {Elements of Information Theory},
 year = {2006},
 isbn = {0471241954},
 publisher = {Wiley-Interscience},
} 

@inproceedings{ternary_quant,
  title={Trained Ternary Quantization},
  author={Zhu, Chenzhuo and Han, Song and Mao, Huizi and Dally, William J},
  booktitle={ICLR},
  year={2017}
}

@inproceedings{imagenet,
AUTHOR = {Jia Deng and Wei Dong and Richard Socher and Li-Jia Li and {Kai Li} and {Li Fei-Fei}},
TITLE = {{ImageNet: A Large-Scale Hierarchical Image Database}},
BOOKTITLE = {CVPR},
YEAR = {2009},
pages={248-255}
}
        

@TECHREPORT{cifar10,
    author = {Alex Krizhevsky},
    title = {Learning multiple layers of features from tiny images},
    institution = {University of Toronto},
    year = {2009}
}

@INPROCEEDINGS{8099498, 
author={X. Yu and T. Liu and X. Wang and D. Tao}, 
booktitle={CVPR}, 
title={On Compressing Deep Models by Low Rank and Sparse Decomposition}, 
year={2017}, 
}

@article{dorefa,
  author    = {Shuchang Zhou and Yuxin Wu and Zekun Ni and Xinyu Zhou and He Wen and Yuheng Zou},
  title     = {{DoReFa-Net: Training Low Bitwidth Convolutional Neural Networks with Low Bitwidth Gradients}},
  journal   = {CoRR},
  volume    = {abs/1606.06160},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.06160},
}

@inproceedings{guidedQuantize,
  title={{Towards Effective Low-Bitwidth Convolutional Neural Networks}},
  author={Bohan Zhuang and Chunhua Shen and Mingkui Tan and Lingqiao Liu and Ian D. Reid},
  booktitle={CVPR},
  year={2018},
  pages={7920--7928},
}


@inproceedings{spectralnet,
title={SpectralNet: Spectral Clustering using Deep Neural Networks},
author={Uri Shaham and Kelly Stanton and Henry Li and Ronen Basri and Boaz Nadler and Yuval Kluger},
booktitle={ICLR},
year={2018},
}

@incollection{rank_manifold,
title = {Ranking on Data Manifolds},
author = {Zhou, Dengyong and Weston, Jason and Gretton, Arthur and Bousquet, Olivier and Sch\"{o}lkopf, Bernhard},
booktitle = {NIPS},
year = {2004},
}

@article{diff_web,
author = {Page, Lawrence and Brin, Sergey and Motwani, Rajeev and Winograd, Terry},
year = {1998},
month = {11},
title = {The PageRank Citation Ranking: Bringing Order to the Web}
}

@INPROCEEDINGS{diff_revisit, 
author={M. Donoser and H. Bischof}, 
booktitle={CVPR}, 
title={Diffusion Processes for Retrieval Revisited}, 
year={2013}, 
}

@inproceedings{diff_orig,
author = {Zhou, Dengyong and Bousquet, Olivier and Lal, Thomas Navin and Weston, Jason and Sch\"{o}lkopf, Bernhard},
title = {Learning with Local and Global Consistency},
booktitle = {NIPS},
year = {2003},
location = {Whistler, British Columbia, Canada},
} 


@ARTICLE{DRSCH, 
author={R. Zhang and L. Lin and R. Zhang and W. Zuo and L. Zhang}, 
journal={IEEE TIP}, 
title={Bit-Scalable Deep Hashing With Regularized Similarity Learning for Image Retrieval and Person Re-Identification}, 
year={2015}, 
volume={24}, 
number={12}, 
}

@inproceedings{hashnet,
title={HashNet: Deep Learning to Hash by Continuation},
author={Cao, Zhangjie and Long, Mingsheng and Wang, Jianmin and Yu, Philip S},
booktitle = {CVPR},
year={2018}
}

@inproceedings{doersch2015unsupervised,
  title = {Unsupervised Visual Representation Learning by Context Prediction},
  author = {Doersch, Carl and Gupta, Abhinav and Efros, Alexei A.},
  booktitle = {ICCV},
  year = {2015}
}

@inproceedings{pathakCVPR16context,
    Author = {Pathak, Deepak and
    Kr\"ahenb\"uhl, Philipp and
    Donahue, Jeff and
    Darrell, Trevor and
    Efros, Alexei},
    Title = {Context Encoders:
    Feature Learning by Inpainting},
    booktitle = {CVPR},
    Year = {2016}
}

@article{FM_gan,
  title={Adversarial Text Generation via Feature-Mover's Distance},
  author={Liqun Chen and Shuyang Dai and Chenyang Tao and Dinghan Shen and Zhe Gan and Haichao Zhang and Yizhe Zhang and Lawrence Carin},
  booktitle={NIPS},
  year={2018}
}

@inproceedings{BGAN,
  title={Binary Generative Adversarial Networks for Image Retrieval},
  author={Jingkuan Song and Tao He and Lianli Gao and Xing Xu and Alan Hanjalic and Heng Tao Shen},
  booktitle={AAAI},
  year={2018}
}

@InProceedings{codes,
author="Douze, Matthijs
and J{\'e}gou, Herv{\'e}
and Perronnin, Florent",
editor="Leibe, Bastian
and Matas, Jiri
and Sebe, Nicu
and Welling, Max",
title="Polysemous Codes",
booktitle="ECCV",
year="2016",
}



@incollection{DGH,
title = {Discrete Graph Hashing},
author = {Liu, Wei and Mu, Cun and Kumar, Sanjiv and Chang, Shih-Fu},
booktitle = {NIPS},
year = {2014},
}

@INPROCEEDINGS{FSH, 
author={H. Liu and R. Ji and Y. Wu and F. Huang and B. Zhang}, 
booktitle={CVPR}, 
title={Cross-Modality Binary Code Learning via Fusion Similarity Hashing}, 
year={2017},}

@article{NSS,
title = "Beyond diffusion process: Neighbor set similarity for fast re-ranking",
journal = "Information Sciences",
volume = "325",
year = "2015",
author = "Xiang Bai and Song Bai and Xinggang Wang",
}

@inproceedings{AnchorGraph,
 author = {Liu, Wei and He, Junfeng and Chang, Shih-Fu},
 title = {Large Graph Construction for Scalable Semi-supervised Learning},
 booktitle = {ICML},
 year = {2010},
} 


@INPROCEEDINGS{ACQ, 
author={G. Irie and H. Arai and Y. Taniguchi}, 
booktitle={ICCV}, 
title={Alternating Co-Quantization for Cross-Modal Hashing}, 
year={2015}, 
}

@inproceedings{MPEC,
  title={An Exact Penalty Method for Binary Optimization Based on {MPEC} Formulation},
  author={Ganzhao Yuan and Bernard Ghanem},
  booktitle={AAAI},
  year={2017}
}

@article{FW,
author = {Frank, Marguerite and Wolfe, Philip},
title = {An algorithm for quadratic programming},
journal = {Naval Research Logistics Quarterly},
volume = {3},
number = {1‐2},
year={1956},
}

@article{FW_convergence,
author = {Lacoste-Julien, Simon},
year = {2016},
month = {07},
title = {Convergence Rate of {F}rank-{W}olfe for Non-Convex Objectives}
}

@inproceedings{ACMR,
 author = {Wang, Bokun and Yang, Yang and Xu, Xing and Hanjalic, Alan and Shen, Heng Tao},
 title = {Adversarial Cross-Modal Retrieval},
 booktitle = {ACM Multimedia},
 year = {2017},
} 

@inproceedings{CVH,
 author = {Kumar, Shaishav and Udupa, Raghavendra},
 title = {Learning Hash Functions for Cross-view Similarity Search},
 booktitle = {IJCAI},
 year = {2011},
} 

@article{CMFH,
  title={Large-Scale Cross-Modality Search via Collective Matrix Factorization Hashing},
  author={Guiguang Ding and Yuchen Guo and Jile Zhou and Yue Gao},
  journal={IEEE TIP},
  year={2016},
  volume={25},
}

@InProceedings{PDH,
  title = 	 {Predictable Dual-View Hashing},
  author = 	 {Mohammad Rastegari and Jonghyun Choi and Shobeir Fakhraei and Daume Hal and Larry Davis},
  booktitle = 	 {ICML},
  year = 	 {2013},
}

@inproceedings{MIRFlickr25k,
 author = {Mark J. Huiskes and Michael S. Lew},
 title = {The {MIR F}lickr Retrieval Evaluation},
 booktitle = {ACM International Conference on Multimedia Information Retrieval},
 year = {2008},
 }

@INPROCEEDINGS{nuswide,
    author = {Tat-seng Chua and Jinhui Tang and Richang Hong and Haojie Li and Zhiping Luo and Yantao Zheng},
    title = {{NUS-WIDE: A} real-world web image database from {N}ational {U}niversity of {S}ingapore},
    booktitle = {CIVR},
    year = {2009}
}

@INPROCEEDINGS{CMDVH,
author={V. E. Liong and J. Lu and Y. Tan and J. Zhou}, 
booktitle={ICCV}, 
title={Cross-Modal Deep Variational Hashing}, 
year={2017}, 
}

@INPROCEEDINGS{DCMH, 
author={Q. Jiang and W. Li}, 
booktitle={CVPR}, 
title={Deep Cross-Modal Hashing}, 
year={2017}, 
month={July},
}

@INPROCEEDINGS{SSAH,
author = {Li, Chao and Deng, Cheng and Li, Ning and Liu, Wei and Gao, Xinbo and Tao, Dacheng},
year = {2018},
booktitle={CVPR}, 
title = {Self-Supervised Adversarial Hashing Networks for Cross-Modal Retrieval}
}

@ARTICLE{SADH, 
author={F. Shen and Y. Xu and L. Liu and Y. Yang and Z. Huang and H. T. Shen}, 
journal={IEEE TPAMI}, 
title={Unsupervised Deep Hashing with Similarity-Adaptive and Discrete Optimization}, 
year={2018}, 
}

@InProceedings{UH-BDNN,
author={Do, Thanh-Toan and Doan, Anh-Dzung and Cheung, Ngai-Man},
title={Learning to Hash with Binary Deep Neural Network},
booktitle={ECCV},
year={2016},
}


@article{ITQ,
  author    = {Yunchao Gong and Svetlana Lazebnik and Albert Gordo and Florent Perronnin},
  title     = {Iterative Quantization: {A} Procrustean Approach to Learning Binary Codes for Large-Scale Image Retrieval},
  journal   = {IEEE TPAMI},
  volume={35}, 
  number={12},
  year      = {2013},
}

@InProceedings{BA,
author = {Carreira-Perpinan, Miguel A. and Raziperchikolaei, Ramin},
title = {Hashing With Binary Autoencoders},
booktitle = {CVPR},
year = {2015}
}

@inproceedings{glove,
  title={Glove: Global vectors for word representation},
  author={Pennington, Jeffrey and Socher, Richard and Manning, Christopher},
  booktitle={EMNLP},
  year={2014}
}



@inproceedings{word2vec,
  title={Efficient estimation of word representations in vector space},
  author={Mikolov, Tomas and Chen, Kai and Corrado, Greg and Dean, Jeffrey},
  booktitle={ICLR Workshop},
  year={2013}
}

@inproceedings{IMH,
 author = {Song, Jingkuan and Yang, Yang and Yang, Yi and Huang, Zi and Shen, Heng Tao},
 title = {Inter-media Hashing for Large-scale Retrieval from Heterogeneous Data Sources},
 booktitle = {ACM SIGMOD},
 year = {2013},
} 

@inproceedings{SpH,
  author    = {Yair Weiss and
               Antonio Torralba and
               Robert Fergus},
  title     = {Spectral Hashing},
  booktitle = {NIPS},
  year      = {2008},
}

@inproceedings{look_imagine_match,
  title={Look, Imagine and Match: Improving Textual-Visual Cross-Modal Retrieval with Generative Models},
  author={Gu, Jiuxiang and Cai, Jianfei and Joty, Shafiq and Niu, Li and Wang, Gang},
  booktitle={CVPR},
  year={2018}
}

@inproceedings{DVSH,
 author = {Cao, Yue and Long, Mingsheng and Wang, Jianmin and Yang, Qiang and Yu, Philip S.},
 title = {Deep Visual-Semantic Hashing for Cross-Modal Retrieval},
 booktitle = {ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
 year = {2016},
} 

@article{VGG,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@inproceedings{LSMVSC,
 author = {Li, Yeqing and Nie, Feiping and Huang, Heng and Huang, Junzhou},
 title = {Large-scale Multi-view Spectral Clustering via Bipartite Graph},
 booktitle = {AAAI},
  year = {2015},
}

@ARTICLE{SSDH, 
author={H. Yang and K. Lin and C. Chen}, 
journal={IEEE TPAMI}, 
title={Supervised Learning of Semantics-Preserving Hash via Deep Convolutional Neural Networks}, 
year={2018}, 
volume={40}, 
number={2}, 
}

@ARTICLE{DH_TIP, 
author={J. Lu and V. E. Liong and J. Zhou}, 
journal={IEEE TIP}, 
title={Deep Hashing for Scalable Image Search}, 
year={2017}, 
volume={26}, 
number={5}, }


@INPROCEEDINGS{SKH, 
author={W. Liu and J. Wang and R. Ji and Y. Jiang and S. Chang}, 
booktitle={CVPR}, 
title={Supervised hashing with kernels}, 
year={2012}, 
}

@ARTICLE{KLSH, 
author={B. Kulis and K. Grauman}, 
journal={IEEE TPAMI}, 
title={Kernelized Locality-Sensitive Hashing}, 
year={2012}, 
}

@book{chung1997spectral,
  title={Spectral graph theory},
  author={Chung, Fan RK and Graham, Fan Chung},
  number={92},
  year={1997},
  publisher={American Mathematical Soc.}
}

@INPROCEEDINGS{AMMSS, 
author={X. Cai and F. Nie and W. Cai and H. Huang}, 
booktitle={ICCV}, 
title={Heterogeneous Image Features Integration via Multi-modal Semi-supervised Learning Model}, 
year={2013}, 
}

@inproceedings{graphHashing,
 author = {Liu, Wei and Wang, Jun and Kumar, Sanjiv and Chang, Shih-Fu},
 title = {Hashing with Graphs},
 booktitle = {ICML},
 year = {2011},
} 

@INPROCEEDINGS{MSRC, 
author={X. Cai and F. Nie and H. Huang and F. Kamangar}, 
booktitle={CVPR}, 
title={Heterogeneous image feature integration via multi-modal spectral clustering}, 
year={2011}, 
}

@article{adagrad,
 author = {Duchi, John and Hazan, Elad and Singer, Yoram},
 title = {Adaptive Subgradient Methods for Online Learning and Stochastic Optimization},
 journal = {J. Mach. Learn. Res.},
 volume = {12},
 year = {2011},
} 

@article{adam,
author = {Kingma, Diederik and Ba, Jimmy},
year = {2014},
title = {Adam: A Method for Stochastic Optimization},
journal = {ICLR}
}

@article{nocedal2006numerical,
  title={Numerical optimization},
  author={Nocedal, Jorge and Wright, Stephen},
  journal={Springer series in operations research, New York, USA},
  year={2006}
}

@incollection{co_reg_MVSC,
title = {Co-regularized Multi-view Spectral Clustering},
author = {Kumar, Abhishek and Rai, Piyush and Hal Daume},
booktitle = {NIPS},
year={2011},
}

@article{CCA,
author = {Hardoon, David R. and Szedmak, Sandor and Shawe-Taylor, John},
title = {Canonical Correlation Analysis: An Overview with Application to Learning Methods},
journal = {Neural Computation},
volume = {16},
number = {12},
year = {2004},
}

@article{cross_retrieval_survey,
  author    = {Kaiye Wang and
               Qiyue Yin and
               Wei Wang and
               Shu Wu and
               Liang Wang},
  title     = {A Comprehensive Survey on Cross-modal Retrieval},
  journal   = {CoRR},
  volume    = {abs/1607.06215},
  year      = {2016},
}

@article{2stephash,
  title={A General Two-Step Approach to Learning-Based Hashing},
  author={Guosheng Lin and Chunhua Shen and David Suter and Anton van den Hengel},
  journal={ICCV},
  year={2013},
}

@inproceedings{SelfTaughtHF,
  title={Self-Taught Hashing for Fast Similarity Search},
  author={Dell Zhang and Jun Wang and Deng Cai and Jinsong Lu},
  booktitle={SIGIR},
  year={2010}
}

@inproceedings{DDCMH,
	author = {Zhen-Duo Chen and Wan-Jin Yu and Chuan-Xiang Li and Liqiang Nie and Xin-Shun Xu},
	title = {Dual Deep Neural Networks Cross-Modal Hashing},
	booktitle = {AAAI},
	year = {2018},
}

@Article{orthogonalProcrustes,
author="Sch{\"o}nemann, Peter H.",
title="A generalized solution of the orthogonal procrustes problem",
journal="Psychometrika",
year="1966",
}

@INPROCEEDINGS{THN,
	author = {Zhangjie Cao and Mingsheng Long and Jianmin Wang and Qiang Yang},
	title = {Transitive Hashing Network for Heterogeneous Multimedia Retrieval},
	booktitle = {AAAI},
	year = {2017},
}

@INPROCEEDINGS{8099765, 
author={D. Mandal and K. N. Chaudhury and S. Biswas}, 
booktitle={CVPR}, 
title={Generalized Semantic Preserving Hashing for N-Label Cross-Modal Retrieval}, 
year={2017}, 
pages={2633-2641}, 
month={July},}

@article{MSAE,
 author = {Wang, Wei and Ooi, Beng Chin and Yang, Xiaoyan and Zhang, Dongxiang and Zhuang, Yueting},
 title = {Effective Multi-modal Retrieval Based on Stacked Auto-encoders},
 journal = {VLDB Endowment},
 issue_date = {April 2014},
 volume = {7},
 number = {8},
 year = {2014},
} 

@ARTICLE{DMHOR, 
author={D. Wang and P. Cui and M. Ou and W. Zhu}, 
journal={IEEE Transactions on Multimedia}, 
title={Learning Compact Hash Codes for Multimodal Representations Using Orthogonal Deep Structure}, 
year={2015}, 
volume={17}, 
number={9}, 
}

@inproceedings{LSSH,
 author = {Zhou, Jile and Ding, Guiguang and Guo, Yuchen},
 title = {Latent Semantic Sparse Hashing for Cross-modal Similarity Search},
 booktitle = {ACM SIGIR},
 year = {2014},
} 

@inproceedings{SAH,
  author    = {Thanh{-}Toan Do and
               Dang{-}Khoa Le Tan and
               Trung T. Pham and
               Ngai{-}Man Cheung},
  title     = {Simultaneous Feature Aggregating and Hashing for Large-scale Image Search},
  booktitle = {CVPR},
  year = {2017},
}

@ARTICLE{DBRC, 
author={D. Hu and F. Nie and X. Li}, 
journal={IEEE Transactions on Multimedia}, 
title={Deep Binary Reconstruction for Cross-modal Hashing}, 
year={2018}, 
}

@INPROCEEDINGS{CMCQ, 
author={T. Zhang and J. Wang}, 
booktitle={CVPR}, 
title={Collaborative Quantization for Cross-Modal Similarity Search}, 
year={2016}, 
}

@inproceedings{CorrAE,
 author = {Feng, Fangxiang and Wang, Xiaojie and Li, Ruifan},
 title = {Cross-modal Retrieval with Correspondence Autoencoder},
 booktitle = {ACM Multimedia},
 year = {2014},
} 

@article{SpectralClusterTutorial,
  title={A tutorial on spectral clustering},
  author={Von Luxburg, Ulrike},
  journal={Statistics and computing},
  volume={17},
  number={4},
  pages={395--416},
  year={2007},
  publisher={Springer}
}

@ARTICLE{SMFH, 
author={J. Tang and K. Wang and L. Shao}, 
journal={IEEE Transactions on Image Processing}, 
title={Supervised Matrix Factorization Hashing for Cross-Modal Retrieval}, 
year={2016}, 
volume={25}, 
number={7}, 
}

@inproceedings{alexnet,
 author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E.},
 title = {ImageNet Classification with Deep Convolutional Neural Networks},
 booktitle = {NIPS},
 year = {2012},
 pages = {1097--1105},
} 

@INPROCEEDINGS{resnet, 
author={Kaiming He and Xiangyu Zhang and Shaoqing Ren and Jian Sun}, 
booktitle={CVPR}, 
title={{Deep Residual Learning for Image Recognition}}, 
year={2016}, 
pages={770--778}
}

@misc{tensorflow,
title={ {TensorFlow}: Large-Scale Machine Learning on Heterogeneous Systems},
url={https://www.tensorflow.org/},
note={Software available from tensorflow.org},
author={
    Mart\'{\i}n~{Abadi}  and others
    },
  year={2015},
}

@misc{tensorpack,
  title={Tensorpack},
  author={Wu, Yuxin and others},
  howpublished={\url{https://github.com/tensorpack/}},
  year={2016}
}
